CHEF: A Cheap and Fast Pipeline for Iteratively Cleaning Label Uncertainties (Technical Report)

High-quality labels are expensive to obtain for many machine learning tasks, such as medical image classification tasks. Therefore, probabilistic (weak) labels produced by weak supervision tools are used to seed a process in which influential samples with weak labels are identified and cleaned by several human annotators to improve the model performance. To lower the overall cost and computational overhead of this process, we propose a solution called CHEF (CHEap and Fast label cleaning), which consists of the following three components. First, to reduce the cost of human annotators, we use Infl, which prioritizes the most influential training samples for cleaning and provides cleaned labels to save the cost of one human annotator. Second, to accelerate the sample selector phase and the model constructor phase, we use Increm-Infl to incrementally produce influential samples, and DeltaGrad-L to incrementally update the model. Third, we redesign the typical label cleaning pipeline so that human annotators iteratively clean smaller batch of samples rather than one big batch of samples. This yields better over all model performance and enables possible early termination when the expected model performance has been achieved. Extensive experiments show that our approach gives good model prediction performance while achieving significant speed-ups.

==> Sections/Response.tex <==
\onecolumn
% \renewcommand\thesection{\Alph{section}}
\setcounter{section}{0}

\section{Response to Reviewer Comments}

\subsection{Response to Reviewer 1}


\textbf{W1}. \textit{The experiments are based on synthetic probabilistic labels, which may not be sufficient to validate the effectiveness of the proposed methods. }

\noindent
\textbf{Response}: We agree with you about your concerns on the lack of datasets with real probabilistic labels. To remedy this, we added three crowdsourced datasets, i.e. \fashion\ dataset, \twitter\ dataset and \fact\ dataset, in the current version of the paper. To produce the probabilistic labels for those datasets, we employ the solution from \cite{boecking2020interactive} to {\bf automatically} derive the labeling functions and thus the probabilistic labels for the \fashion\ dataset and \twitter\ dataset, and follow the labeling functions from \cite{chatterjee2019data} to produce probabilistic labels for \fact\ dataset. But we note that the solutions to automatically generate labeling functions and probabilistic labels are not mature at this moment for the pure image dataset, e.g. \retina, \mimic\ and \chexpert\ dataset. Therefore, we still employ the synthetic probabilistic labels for.those three datasets. In the end, we found that our methods can outperform the baseline methods in most cases for those six datasets, thus justifying the effectiveness of our methods.

\noindent
\textbf{W2}. \textit{The improvement of the label cleaning seems not significant, and more method comparisons are needed.}

\noindent
\textbf{Response}: We agree that the improvement of the label cleaning is not significant. The main reason is that the probabilistic labels may hurt the model performance, but earlier we weighted all the training samples (with deterministic labels or probabilistic labels) equally. In practice, as you pointed out, it is reasonable to regularize on the samples with probabilistic labels (e.g. see \cite{sukhbaatar2014learning}). We therefore take this into consideration in our method. 
% It turns out that after downweighting the training samples with probabilistic labels, the improvement of the label cleaning becomes more significant. 
We also compare \infl\ against more baseline methods in varied experimental settings, e.g. different models, different regularization rate on the training samples with probabilistic labels. The results indicate that \infl\ performs better in almost all the scenarios.

\noindent
\textbf{W3}: \textit{More related studies on data annotation should be discussed.}

\noindent
\textbf{Response}: Done

\noindent
\textbf{D1}. \textit{Overall, this is a well-organized SDS paper based on solid work. Although the framework seems not new, the paper introduces new techniques in both sample selector and model parameter updating phases.}

\noindent
\textbf{Response}: Thanks for your comments. We agree that the overall label cleaning framework may not be new. However, as you mentioned, we proposed some new techniques in the sample selection phase, the model construction phase and the human annotation phase for reducing their time overhead and the labeling cost, which are the main contribution of this paper.

\noindent
\textbf{D2}. \textit{The authors claim in the Introduction that "To produce labels at a much larger scale with lower cost, weak supervision tools, such as the labeling functions in Snorkel \cite{ratner2017snorkel}, can be used to automatically generate probabilistic labels for unlabeled training samples". However, in the experiments, the authors use a very simple strategy to generate probabilistic labels: "select 70\% of the training samples and replace their labels with randomly generated probabilistic labels". I do not think this experimental setting is sufficient to validate the effectiveness of the proposed methods. I suggest the authors to consider real datasets with probabilistic labels. For example, some existing studies directly use crowdsourced labels as inaccurate labels.}

\noindent
\textbf{Response}: Thanks for pointing this out. As you suggested, we added experiments on three real datasets with crowdsourced labels, i.e. the Fashion 10000 dataset\footnote{\url{http://skuld.cs.umass.edu/traces/mmsys/2014/user05.tar}}, Fact Evaluation Judgement dataset\footnote{ \url{https://sites.google.com/site/crowdscale2013/shared-task/task-fact-eval}} and Twitter sentiment analysis dataset\footnote{\url{https://github.com/naimulhuq/Capstone/blob/master/Data/Airline-Full-Non-Ag-DFE-Sentiment\%20(raw\%20data).csv}}. You can find the brief descriptions of the three datasets in our paper. But those three datasets do not have any probabilistic labels or any labeling functions.
To deal with this, we leverage some recent work (such as \cite{boecking2020interactive, varma2018snuba}) from the ML community to automatically generate the labeling functions and thus the probabilistic labels based on the text data in those three datasets. But we still produce the random probabilistic labels for retina, mimic and chexpert datasets since no labeling functions are available for those three datasets and also the existing tools are not capable of automatically producing probabilistic labels for such large image datasets without any text information. We will consider repeating our current experiments in the future for those three datasets once we can obtain realistic probabilistic labels for them.


\noindent
\textbf{D3}. \textit{Observed from Table 2, the improvement on F1 is not significant. Moreover, it would be better if the authors to compare more baselines. For example, how about using a deep learning model, such as CNN, with regularization on the probabilistic labels? Will this method achieve comparable performance with Strategy two?}

\noindent
\textbf{Response}: Thanks for your suggestions on comparing our method against deep learning models with regularization on the probabilistic labels. To address your concerns on this, first of all, we modified our method, \infl, such that it can take the regularization on the probabilistic labels into consideration. We also clarify in the paper that \infl\ is actually not limited to simple models. Instead, it is applicable for any complicated models. As a result, rather than comparing CNN+regularization against strategy two, we added one experiment in Appendix \ref{sec: exp_cnn_model} to show how \infl\ performs when CNN+regularization is used. The results indicate that \infl\ can still outperform other methods.

\noindent
\textbf{D4}. \textit{It would be better if the authors further compare with more related studies on label cleaning and data annotation. Some are listed as follows.
- Mohamad Dolatshah, Mathew Teoh, Jiannan Wang, Jian Pei: Cleaning Crowdsourced Labels Using Oracles For Statistical Classification. Proc. VLDB Endow. 12(4): 376-389 (2018).
- Jingru Yang, Ju Fan, Zhewei Wei, Guoliang Li, Tongyu Liu, Xiaoyong Du: Cost-Effective Data Annotation using Game-Based Crowdsourcing. Proc. VLDB Endow. 12(1): 57-70 (2018)}

\noindent
\textbf{Response}: Thanks for the suggestion on comparing with those recently published label cleaning methods. In the modified paper, we choose to compare our method against \tars\ from the first paper above (i.e. the one titled ‘Cleaning Crowdsourced Labels Using Oracles For Statistical Classification’). This paper has similar settings to ours since both of our work target the label cleaning tasks for ML models. But we note that \tars\ is only applicable for the scenario where the noisy labels are 0 or 1 rather than probabilistic labels. In contrast, our method can deal with more general settings where the noisy labels are probabilistic labels, including the extreme cases where all the noisy labels are deterministic. To facilitate the fair comparison between our method and \tars, we round the probabilistic labels to the nearest deterministic labels such that both our method and \tars\ can be applied. Due to the space limit, the results for this experiment are included in Appendix \ref{sec: exp_tars}, which shows that our method can outperform \tars. Since our method can also deal with more general scenarios, we can thus expect that our method is more favorable in practice.

\noindent		
However, we did not use the method from the second paper above (i.e. the one titled as Cost-Effective Data Annotation using Game-Based Crowdsourcing) since it only focuses on the entity matching applications and the rule-based models.

\noindent
\textbf{R2}. \textit{It would be better if the author provide supplemental material for reproducibility.}

\textbf{Response}: \textbf{Response}: As claimed in Section \ref{sec: exp}, we released our code in \url{https://github.com/thuwuyinjun/Chef}.



\subsection{Response to Reviewer 2}

\noindent
\textbf{W1}: \textit{Limited novelty and technical motivation.}

\noindent
\textbf{Response}: We understand that not all the components of our solutions are new. However, since this is the scalable data science track, according to the submission guidelines, this type of submission could be ``showing success of adaptations of recent techniques in helping solve an important and practical data science problem''. In this paper, we adapted our previous solution on incrementally maintaining ML models, i.e., \deltagrad, for speeding up the label cleaning applications. We also proposed \deltagradg\ for incrementally identifying the influential training samples for label cleaning, which can make the entire label cleaning pipeline more scalable. To justify the feasibility of our solution, we evaluate it on several realistic datasets, including the ones with real crowdsourced labels.

\noindent
\textbf{W2}: \textit{The impact of using samples with uncertain labels in training is not clear.}

\noindent
\textbf{Response}: We agree that the uncertain labels on the training samples may lead to negative effects on the model quality. To regularize such possible negative effects, we follow \cite{sukhbaatar2014learning} to down-weight the training samples with uncertain labels and we also extend our method to take such regularization into account. 

\noindent
\textbf{W3}: \textit{The comparison/motivation with regard to alternative approaches such as AL (with uncertainty sampling) is not clear.}

\noindent
\textbf{Response}: Thanks for your suggestion on comparing our solution against the active learning methods. In the modified paper, we extensively compare our method against two variants of uncertainty-based active learning methods, i.e. the least confidence based sampling method and the entropy based sampling method. The results show that in almost all the scenarios, our method can beat the active learning methods. As mentioned above, we add the regularization on the training samples with uncertain labels. So note that when the regularization rate, i.e. the weight on the training samples with uncertain labels, is 0, it is the same as the classical set-up for the active learning methods. We therefore also compare our method against AL in this set-up and again demonstrate the performance advantages of our method in most datasets. Plus, since our method can fully rely on the automatically derived labels rather than the human annotated labels, it can thus also be helpful in reducing the human annotation cost with respect to active learning methods.

\noindent
\textbf{W4}: \textit{Experiments simulate human annotators, hence miss to evaluate their impact in the framework.}

\noindent
\textbf{Response}: We agree that the previous version of the paper fails to evaluate our solutions in the presence of real human annotators. To remedy this problem, we use three realistic crowdsourced datasets with crowdsourced labels from different human annotators, i.e. Fashion dataset, Fact dataset and twitter dataset. We can show that by using the automatically generated labels from our method, the model performance can be even better than that with only human annotated labels. This can thus demonstrate that it is reasonable to regard the automatically generated labels as one independent labeler in practice for reducing the human annotation cost.

\noindent
\textbf{D1} \textit{Why not simply applying active learning with uncertainty sampling over the unlabeled pool and choose the most uncertain outcomes (e.g. max entropy) for labeling? At a high level, why the proposed work in this paper different/better than this?}

\noindent
\textbf{Response}: First of all, we have modified our method such that it can regularize the training samples with uncertain labels and thus reduce the possibly negative effect brought by the uncertain labels, which is the same as the set-up proposed in \cite{sukhbaatar2014learning}. Therefore, we can know that when the regularization rate (i.e., the weight on the training samples with uncertain labels) is zero, it will be the same as the classical settings for the active learning methods, where unlabeled or uncleaned training samples are not involved in the model training process. On the other hand, when the regularization rate is one, it will be the same as the settings for weak supervised learning. As a result, by comparing against the classical active learning methods, our method for cleaning uncertain labels can be suitable for more general scenarios.

% \noindent
Second, in the modified version of the paper, we also conduct the experiments to compare our method and the active learning methods in cleaning the uncertain labels under different scenarios, e.g. with varied regularization rate on the training samples with uncertain labels. For fair comparison between those two types of methods, we use the same objective function for training the model, i.e. the one regularizing the training samples with uncertain labels. According to the experimental results, in almost all the scenarios across different datasets, our method outperforms the active learning methods. Intuitively speaking, our method selects the most influential training samples by quantifying \textbf{how the model performance is improved} after the label of one training sample is cleaned. In contrast, active learning methods select the most influential training samples through the prediction uncertainties or the entropy, which may fail when the model performance is not ideal.


\noindent
\textbf{D2} \textit{The paper proposes to show a subset of top-b (less than B) to the user for labeling. How is b identified? In particular, how is it better than the sequential labeling used in traditional active learning settings?}

\noindent
\textbf{Response}: First of all, using a subset of cleaning budget, i.e. $b$, has two benefits. The first benefit is that the human annotators can interact with the Sample selector for multiple times and early termination is possible with smaller $b$. The other (more important) benefit is that better model performance can be achieved with smaller $b$. Recall that the influence function estimates the influence of one sample rather than the joint effect of multiple samples. Therefore, with larger $b$, the joint effect of a large set of training samples may be ignored by the influence function, thus leading to sub-optimal solutions. To illustrate this effect, we evaluate the model performance with varied sizes of $b$ in the experiments and the experimental results can demonstrate the above benefit by using small $b$. Similar phenomena appear when active learning methods are used.


But note that smaller $b$ means more rounds to clean the uncertain labels, thus increasing the overall running time. As a result, we would expect a medium size of $b$ to balance the model performance and the running time. To illustrate this, we compared the model performance and the running time with varied $b$ in Appendix \ref{sec: vary_b} and found that setting $b$ as around 10\% of the cleaning budget would be a reasonable choice.


\noindent
\textbf{D3} \textit{Compared to the existing work \cite{krishnan2016activeclean} this paper proposes to still use the probabilistic labels for learning but to make sure those are not "high impact". This, to me sounds a little bit confusing: (a) if the probabilistic labels are not impactful, why bother to use them in training? (b) if those are impactful how do you know if your outcome model is accurate.
The authors try to identify the impactful probabilistic samples and label them. But again it takes me back to my original point that if the points that are not labeled (after exhausting the budget B) are not impactful, why bothering to use them in training.}

\noindent
\textbf{Response}: We agree that depending on different datasets, the probabilistic labels may have varied effects on the model performance. It is possible that the probabilistic labels may have negative effects on the model quality. Therefore, we follow \cite{sukhbaatar2014learning} to regularize the training samples with uncertain labels such that their possibly negative could be reduced. However, {\em we do not assume that the probabilistic labels are not highly impactful or not}. We even demonstrate the performance advantage of infl with varied regularization rate, which can lead to different impacts brought by the probabilistic labels. But as our experiments indicate, our methods can lead to better model performance than the active learning methods after the same number of training samples are cleaned in almost all scenarios. This is because when infl is used to select the most influential training samples, it does not depend on the model performance. Instead, it relies on how cleaning those influential training samples improves the model performance, which can be estimated by using the influence function no matter what the model performance is before or after the label cleaning operations.

\noindent
\textbf{D4} \textit{This takes me to my next argument, that even after exhausting the budget B, what is left as uncertain labels can still have an {\em aggregate impact} that dominates the aggregate impact of deterministic labels. It of course depends on the labeling budget and the ratio of uncertain labels to deterministic ones. To see why, let all uncertain labels be a single "uncertain" player. Now, the Shapley value of this uncertain player show the aggregate impact of this player compared to other players (each being a deterministic label). It is easy to see that depending on the number of uncertain labels, their aggregate impact as the uncertain player can dominate the deterministic labels and generate an inaccurate outcome. It is not clear how this has been measured/prevented in the paper.}

\noindent
\textbf{Response}: Thanks for your concerns on this point. As we mentioned above, it is possible that the uncertain labels can lead to worse model performance. Therefore, we follow \cite{sukhbaatar2014learning} to regularize those samples during the model training phase and adjust our methods accordingly. Plus, our method, \infl, does not depend on the model performance. Instead, it depends on how cleaning the influential training samples improve the model performance, which can be estimated with the influence function. Our latest experimental results show that \infl\ can help improve the model performance most with respect to other baseline methods, including active learning methods.


\noindent
\textbf{D5} \textit{The technical contribution of this paper is limited and it is mostly applying existing techniques, including the previous work by authors for speeding up the sample-labeling determination.}

\noindent
\textbf{Response}: As mentioned above, the scalable data science paper aims at “showing success of adaptations of recent techniques in helping solve an important and practical data science problem”. Therefore, we think that adapting our previous work for the label cleaning problem could be a good fit for this type of submission.

\noindent
\textbf{D6} \textit{I believe the human labeling time should dominate the model reconstruction from scratch. This significantly reduces the impact of model-constructor phase. In other words, if human labeling time is high (which should be the case for costly labeling environments), what do we gain from using an approximate model (in faster time) instead reconstructing the exact model from scratch.}

\noindent
\textbf{Response}: We agree that human labeling time might be the most significant overhead in the overall label cleaning pipeline. However, as we claimed in the paper, given a fixed cleaning budget, our design allows the human annotators to interact with our system for multiple times (with smaller b) such that the model performance could be better than the case when the human annotators use the system for one time. Therefore, when the human annotators interact with our system, it would be essential to make our system as efficient as possible such that they do not have to wait for a long time to get the instruction on which samples to be cleaned at the next round. To achieve this, one option is to speed up the model construction step by using our previous techniques on incrementally updating ML models. 


In addition, as we indicate in the paper, our method, \infl, can also automatically suggest cleaned labels. If we simply use those labels to replace the uncertain labels, i.e. the strategy two (renamed as \cleantwo) in the experiment section, we can achieve the best performance in most cases, especially on the real crowdsourced datasets. Therefore, when high-quality human annotators are not available, \infl\ would be an ideal alternative labeler, which can help us significantly save the human labeling time.

\noindent
\textbf{D7} \textit{Unfortunately, the paper does not use real crowd for experimental evaluations. In particular, this prevented observing the real difficulties of using real crowd and to see how much time it takes for evaluate the label of a sample by multiple users to assure it is correct.}

\noindent
\textbf{Response}: Thanks for your comments on the use of real crowdsourced datasets. First of all, we conduct our experiments on three more real crowdsourced datasets, each of which includes the labels provided by different human annotators. The experimental results show that our method can not only achieve better model prediction performance than other baseline approaches in most cases, but also significantly reduce the running time on model construction step and sample selection step.  


Second, as mentioned above, we agree that human labeling time is the major overhead in the label cleaning process. To reduce this overhead, we evaluate the model performance when we simply use the suggested labels by \infl\ without using any human annotated labels, the best performance could be achieved in most cases. This thus indicates that \infl\ could be a good labeler in practice, thus significantly reducing the human annotation time and cost.


\noindent
\textbf{D8} \textit{The paper uses a subset of labeled points as validation/test sets which is a waste of budget for costly and limited labeled environments. Instead, why not using all labeled samples for training?}

\noindent
\textbf{Response}: We are following the classical machine learning protocol by partitioning the entire dataset into training, validation and test sets. The validation set is used for model selections and the test set is used for evaluating the model performance. We note that in some real crowdsourced datasets, such as \fact\ dataset and \twitter\ dataset, there exist some small number of samples with ground-truth labels. Thus those samples can be used for composing the validation set and test set.



\subsection{Response to Reviewer 3}
\textbf{W1}. \textit{Some important details are not included in the main paper. For example, the time complexity of \deltagradg\ and some detailed experiment setups.}

\noindent
\textbf{Response}: Thanks for your suggestions on including more details in the main paper. As you suggested, we describe the time complexity of \deltagradg\ in Section \ref{sec: sample_selector} and parts of the hyper-parameters in Section \ref{sec: exp_design}. However, different datasets may use different hyper-parameters. Due to the space limit, we have to include all the remaining hyper-parameters in Appendix \ref{appendix-sec: hyper}.

\noindent
\textbf{W2}. \textit{Experiment. The datasets lacks variations, i.e., all three datasets are in the same domain. In addition, there are some basic questions that are not answered by the experiment.}

\noindent
\textbf{Response}: Thanks for your comments. In the latest version of the paper, we run our experiments on three more real crowd-sourced datasets, i.e., \fact\ dataset, \fashion\ dataset and \twitter\ dataset. Among those three datasets, \fact\ and \twitter\ dataset are text dataset while \fashion\ is an image dataset. We can still demonstrate the performance advantage of our method in those three datasets. 

\noindent
\textbf{W3}. \textit{Presentation. Figure 1 looks very busy and the labels are hard to read. Lack of detailed description of the objective function for Increm-Infl (Algorithm 2).}

\noindent
\textbf{Response}: Thanks for pointing those two issues out. To address your first concern, we removed some unnecessary elements and increased the font size in Figure 1 to make it clear. In terms of the second issue, we should clarify that the objective function exists for the method \infl\ but not for the algorithm \deltagradg. Specifically, the goal of using \infl\ is to find out a set of $b$ training samples such that their influence could be {\em maximized} after their labels are cleaned. But instead of iterating all training samples, we proposed \deltagradg\ to reduce the search space, which can thus be regarded as a type of pruning algorithm. Since there is no explicit objective function for classical pruning algorithms, such as Alpha–beta pruning algorithm, then there might be no suitable objective function for \deltagradg. To avoid confusing readers, We explicitly clarified in the beginning of Section \ref{sec: deltagradg} that \deltagradg\ is used for reducing the search space when \infl\ is used.

\noindent
\textbf{D1}. \textit{Experiment dataset. Selection of datasets lacks variation. All the selected datasets are for medical image classification. The proposed solution can also be applied to many data management tasks, e.g., entity matching and error detection.}

\noindent
\textbf{Response}: Thanks for your comments. In the latest version of the paper, we run our experiments on three more real crowd-sourced datasets, i.e., \fact\ dataset, \fashion\ dataset and \twitter\ dataset. Among those three datasets, \fact\ dataset is a text dataset for fact evaluation judgement, \twitter\ is a text dataset for sentimental analysis while \fashion\ is another image dataset. For those three datasets, we can still demonstrate the performance advantage of our method in those three datasets, which indicates the applicability of our method in various applications.

\noindent
\textbf{D2}. \textit{Experiment design. There are some basic questions the authors did not consider in their current experiments. For example, why is it necessary to use Increm-Infl to select examples? E.g., compared to 2000 random examples OR examples with noisy labels, identified by noisy label detection algorithms (via cross validation or more advanced algorithms).}

\noindent
\textbf{Response}: Thanks for pointing this out. As mentioned above, \deltagradg\ is not used for selecting samples directly. Instead, it is used for reducing the search space before the Top-$b$ influential training samples are identified by \infl. To justify the necessity of using \infl\ for selecting the influential training samples, we further compare it against two noisy label detection algorithms, i.e. \ou\ and \tars. The results show that \infl\ could beat those two algorithms in varied scenarios. 

\noindent
\textbf{D3}. \textit{Objective function for the sample selector phase. What is the objective function (formally) for Algorithm 2? }

\noindent
\textbf{Response}: As mentioned above, there is no explicit objective function for Algorithm 2. It is just used for reducing the search space.


==> Sections/conclusion2.tex <==
\vspace{-0.2cm}
\section{Conclusions}\label{sec: conclusion}
\eat{To mitigate the lack of  high-quality labels in medical image classification tasks, weak labels are widely used, which, however, often need to be further cleaned by human annotators to improve model performance. The pipeline of cleaning uncertain labels is typically iterative, consisting of a {\em sample selector phase}, {\em human annotation phase} and  {\em model constructor phase}. To reduce the overall cost and time overhead of each phase of this label cleaning process, }
In this paper, we propose \method, which can reduce the overall cost of the label cleaning pipeline and achieve better model performance than other approaches; it may also allow early termination in the human annotation phase. 
\eat{1) reduce the cost of the human annotation phase through a modified version of the influence function, \infl; 2) decrease the time overhead of the sample selector phase by incrementally identifying the most influential training samples with \deltagradg; and 3) speed up the model constructor phase by incrementally updating the model using \deltagradl. }
Extensive experimental studies show the effectiveness of our solution over a broad spectrum of real datasets when logistic regression models are used.
\eat{show that our approach can guarantee the model prediction performance while achieving significant speed-ups.}
% As the first step toward generalizing our techniques to more general settings, 
We also evaluate the performance of \infl\ for CNN models. 
% (see Appendix \ref{sec: exp_cnn_model}). 
How to extend other components of \method\ beyond strongly convex models is left as future work.
\eat{ One limitation of this work is that other than \infl, it can only support strongly convex models. Exploring how to generalize the above techniques for more advanced ML models is left as the future work.}

\begin{acks}
This material is based upon work that is in part supported by the Defense Advanced Research Projects Agency (DARPA) under Contract No. HR001117C0047.
% Partial support was provided by NSF Awards 1547360 and 1733794.
\end{acks}

==> Sections/experiments2.tex <==
\section{Experiments}\label{sec: exp}
We conducted extensive experiments in Python 3.6  and PyTorch 1.7.0 \cite{paszke2017automatic}. All experiments were conducted on a Linux server with an Intel(R) Xeon(R) CPU E5-2630 v4 @ 2.20GHz, 3 GeForce 2080 Titan RTX GPUs and 754GB of main memory. 
% Code has been released in GitHub\footnote{see https://github.com/thuwuyinjun/Chef}.

\subsection{Experimental setup}\label{sec: exp_setup}
%\textbf{Platform}
%\textbf{Datasets} 
%We experimentally evaluate our methods on t
Two types of datasets are used, one of which is annotated with ground-truth labels but no human generated labels, while the other is fully annotated with crowdsourced labels but only partially annotated by ground-truth labels. The former type (referred to as \textit{\cleanset}) is used to evaluate the quality of  labels suggested by \infl\ by comparing them against the ground-truth labels. The latter type (referred to as \textit{\crowdset}) is used for evaluating the performance of our methods in more realistic settings. The two types of datasets are briefly described next.
\eat{; more detailed descriptions %of the three datasets 
can be found in the extended technical report \cite{wu2021chef}}
% Appendix \ref{appendix_sec: dataset}. 

\cleanset: Three real medical image datasets are used: \mimicfull\ (\mimic\ for short) \cite{johnson2019mimic}, \chexpert\ \cite{irvin2019chexpert} and \retinafull\ (\retina\ for short)  \cite{gulshan2016development}. The datasets are used to identify whether one or more diseases or findings exist for each image sample. In the experiments, we are interested in predicting the existence of findings called ``Lung Opacity'', ``the referable Diabetic Retinopathy'' and ``Cardiomegaly'' for \mimic, \retina\ and \chexpert,  respectively. 



\crowdset: Three realistic crowdsourced datasets are used: \fashionfull\ (\fashion\ for short)\footnote{available at \url{http://skuld.cs.umass.edu/traces/mmsys/2014/user05.tar}} \cite{loni2014fashion}, \factfull\ (\fact\ for short)\footnote{available at \url{https://sites.google.com/site/crowdscale2013/shared-task/task-fact-eval}}, and \twitterfull\ (\twitter\ for short)\footnote{available at \url{https://github.com/naimulhuq/Capstone/blob/master/Data/Airline-Full-Non-Ag-DFE-Sentiment\%20(raw\%20data).csv}}. 
%As claimed above, o
Only a small portion of samples in the datasets have ground-truth labels while the rest are labeled by %multiple realistic 
crowdsourcing workers (e.g., the labels of the \fashion\ dataset are collected through the Amazon Mechanical Turk (AMT) crowdsourcing platform). The \fashion\ dataset is an image dataset for distinguishing fashionable images from unfashionable ones; the \fact\ dataset uses RDF triples to represent facts about public figures and the classification task is to judge whether or not each fact is true; and the \twitter\ dataset consists of plain-text tweets on major US airlines for sentiment analysis, i.e., identifying positive or negative tweets. For the \fashion\ and \fact\ datasets, extra text is also associated with each sample, e.g. user comments on each image in \fashion\ and the evidence for each fact in \fact, which is critical for producing probabilistic labels (see discussion below).




% along with some plain-text evidence from the Wikipedia




% \texttt{\mimic\ dataset}

% \texttt{\retina\ dataset}

% \texttt{\chexpert\ dataset}
% In contrast, the other three datasets are all real medical imaging datasets which only have ground-truth labels without having any human annotated labels. The purpose of using those three datasets in the experiments is to compare the suggested labels by \infl\ against the ground-truth labels to evaluate the equality of those labels. 
%We briefly introduce the six datasets as follows and more detailed descriptions could be found in Appendix \ref{appendix_sec: dataset}. 

Since some samples in the datasets  have missing or unknown %or undetermined labels for the findings mentioned above
ground-truth labels,  %(denoted as -1), 
we remove them in the experiments. Also, except for \mimic\ which has 579 validation samples and 1628 test samples, other datasets do not have well-defined validation and test set. For example, as of the time the experiments were performed, the test samples of \chexpert\ had not been released. To remedy this, we partition the \chexpert\ validation set into two parts to create validation and test sets, each of which have 234 samples. Since there was no validation set for \retina, we randomly select roughly 10\% training samples, i.e., 3512 samples, as the validation set.
% training samples from each of those datasets as the validation samples and consider the original validation set as the test set for \chexpert\ such that the validation set and the test set have roughly the same distributions. 
Similarly, for the \twitter\ and \fact\ datasets, we randomly partition the set of samples with ground-truth labels as the validation set and test set, and regard all the other samples as the training set.
% Plus, the training-validation-test set partitions are not provided for \crowdset. To tackle this, , we randomly partition  
Since ground-truth labels are not available in the \fashion\ dataset, we randomly select roughly 0.5\%\footnote{This ratio is determined based on the observation that in the \twitter\ and \fact\ datasets, the percentage of samples with ground-truth labels is less than 1\% of the size of the entire dataset.} of the sample samples as the validation set and test set, each containing 146 samples. The ``ground-truth'' labels for those samples are determined by aggregating human annotated labels using majority vote. The remaining samples in this dataset are then regarded as training samples. In the end, the six datasets, i.e., \mimic, \retina, \chexpert, \fashion, \fact\ and \twitter\ include $\sim$78k,$\sim$31k,$\sim$38k,$\sim$29k,$\sim$38k and $\sim$12k training samples. 
% More detailed statistics of the six datasets are given in Appendix \ref{appendix_sec: dataset}.
% the other two datasets do not have 


\textbf{Producing probabilistic labels} 
Due to the lack of probabilistic labels or labeling functions \cite{ratner2017snorkel} for the datasets, %one plausible solution is leverage
we can choose to leverage \cite{boecking2020interactive}, \cite{varma2018snuba} or \cite{das2020goggles} to {\em automatically} derive suitable labeling functions and thus probabilistic labels in the experiments.
\eat{Ideally, we expect to employ  the labeling functions \cite{ratner2017snorkel} provided by domain experts for producing probabilistic labels for those six datasets, which, unfortunately are not available. But we note that the labeling functions could be automatically derived, by utilizing such as \cite{boecking2020interactive},\cite{varma2018snuba} and \cite{das2020goggles}, which are utilized producing probabilistic labels in the experiments.}
% on automatically deriving suitable labeling functions, 
% to produce probabilistic labels.
% for both \cleanset\ and \crowdset. 
Note that \cite{boecking2020interactive} and \cite{varma2018snuba} deal with text data (including the text associated with image data) while \cite{das2020goggles} targets pure image data. However, the time and space complexity of \cite{das2020goggles} is quadratic in the dataset size, and does not scale to large image datasets such as our \cleanset. Furthermore, no text information is available for images in \cleanset, so it is not feasible to use \cite{boecking2020interactive} or \cite{varma2018snuba}. As a result, 
% one plausible solution to produce probabilistic labels is to leverage \cite{das2020goggles} for those datasets. Unfortunately, due to some scalability issues in \cite{das2020goggles}, 
random probabilistic labels are produced for  
% , which suffers from some scalability issues after our trials of its implementations. 
% however, depend on the domain knowledge for . The lack of
% As described above, we only retain samples with deterministic labels in the experiments. 
% To produce probabilistic labels for \cleanset, 
% {\em sample selector} pick up the most influential training samples in practice, 
all training samples. For \crowdset, we apply \cite{boecking2020interactive} on the extra text information in \fashion\ (e.g. user comments for each image) and the plain-text tweets in \twitter\ dataset to produce probabilistic labels. For \fact\ dataset, the two texts for each sample (i.e. the RDF triples and the associated evidence) are compared using \cite{chatterjee2019data} to generate labeling functions. 
% In contrast, since text information exists   which are then fed into the pipeline in Figure \ref{fig:pipeline}. 

\textbf{Human annotator setup}
For \crowdset, we can use the crowdsourced labels as the cleaned labels for the uncleaned training samples.
% to label the selected influential training samples by the Sample selector. 
However, such labels are unavailable in \cleanset. To remedy this, we note that the error rate of manually labeling medical images is typically between 3\% and 5\%
, but sometimes can be up to 30\% 
\cite{brady2017error}.
% human annotators may erroneously label  at an error rate
% of , and sometimes up to 30\% , 
We therefore produce synthetic human annotated labels by flipping the ground truth labels of a randomly selected 5\% of the samples 
\footnote{Recall that although the samples have probabilistic labels, their true labels are known by construction.}.
% by following the labeling error rates incurred by the human annotators in practice. 
% Specifically, we notice that,  
%Therefore, in practice multiple human annotators are used in the label cleaning process, and label conflicts are resolved using majority vote (e.g., see \cite{irvin2019chexpert}). In the experiments, we assume that there are three independent
% To simulate a human annotator cleaning a set of samples, 
% We therefore . 
% (the randomly selected samples are independent between the three annotators). 
We assume three independent annotators, and aggregate their labels as the cleaned labels using majority vote (denoted \cleanone).
% One goal of the experiments is to compare \infl\ against other variants of the influence functions and \duti\ \cite{zhang2018training}. 
Since \infl\
% and \duti\ \cite{zhang2018training} 
can suggest cleaned labels, those labels can be used as cleaned labels by themselves for the uncleaned samples 
% we can also consider using those labels 
% the suggested labels to be one of the annotators for those two methods, which can 
% to annotate the uncleaned samples by itself 
(denoted \cleantwo) or be combined with two other simulated human annotators for label cleaning 
(denoted \cleanthree).
% clean the labels of the influential training samples selected by the {\em Sample selector}, 
% the probabilistic labels of those samples are replaced with their original deterministic labels.

\eat{We provide two setups for the model constructor. The first one follows the strong convexity assumption on the ML models, which is to justify the performance advantage of our design as a whole (including \deltagradg, \deltagradl\ and \infl). In this setup, pre-trained models are leveraged for feature transformation and 
% transform the original sample features to some latent representation and 
then a logistic regression model is used for classification, which has emerged as a convention
% This results in acceptable performance 
for medical image classification tasks~\cite{raghu2019transfusion}. 
% For , it is reasonable to leverage pre-trained models to transform the original medical images to some latent representation, and . 
Specifically, in the experiments, we use a pre-trained ResNet50 \cite{he2016deep} for the image datasets (\cleanset\ and \fashion), and use a pre-trained BERT-based transformer \cite{devlin2018bert} for the text datasets (\fact\ and \twitter). Stochastic gradient descent (\sgd) is then used in the subsequent training process with a mini-batch size of 2000, 
% L2 regularization rate ranging from 0.001 to 0.05 (depending on the dataset) 
and weight $\gamma= 0.8$ on the uncleaned samples. Early stopping is also applied to avoid overfitting. Other hyper-parameters for model training are varied across different datasets (see Table \ref{Table: hyper_params}). As discussed in Section \ref{sec: intro}, other than the initialization step, we can construct the models by either retraining from scratch (denoted \retrain) or leveraging \deltagrad\ for incremental updates. 

In the second model constructor setup, we aim at evaluating the performance of \infl\ when neural network models are used. Specifically, for the image datasets such as \mimic\ and \retina, we utilize the LeNet \cite{le1989handwritten} model (a classical convolutional neural network structure) on the original image features while for the text datasets, such as \twitter\ and \fact\ dataset, we utilize the 1D convolutional neural network on the embedding representations after the pre-trained BERT-based transformer is applied on the plain text. }



\textbf{Model constructor setup} 
Throughout the paper we assume that strong convexity holds on the ML models. Therefore, in this section, to justify the performance advantage of our design as a whole (including \deltagradg, \deltagradl\ and \infl), we focus on a scenario where pre-trained models are leveraged for feature transformation and 
% transform the original sample features to some latent representation and 
then a logistic regression model is used for classification, which has emerged as a convention
% This results in acceptable performance 
for medical image classification tasks~\cite{raghu2019transfusion}. 
% For , it is reasonable to leverage pre-trained models to transform the original medical images to some latent representation, and . 
Specifically, in the experiments, we use a pre-trained ResNet50 \cite{he2016deep} for the image datasets (\cleanset\ and \fashion), and use a pre-trained BERT-based transformer \cite{devlin2018bert} for the text datasets (\fact\ and \twitter). 
Stochastic gradient descent (\sgd) is then used in the subsequent training process with a mini-batch size of 2000, 
% L2 regularization rate ranging from 0.001 to 0.05 (depending on the dataset) 
and weight $\gamma= 0.8$ on the uncleaned samples. Early stopping is also applied to avoid overfitting. Other hyper-parameters for model training are varied across different datasets (see Table \ref{Table: hyper_params}). We also vary $\gamma$ for a more extensive comparison in \cite{wu2021chef}.

As discussed in Section \ref{sec: intro}, other than the initialization step, we can construct the models by either retraining from scratch (denoted \retrain) or leveraging \deltagradl\ for incremental updates. For the latter case, 
% When the logistic regression models are incrementally updated using \deltagradl\ 
% (see Algorithm \ref{alg: deltagrad})
the hyper-parameters of \deltagradl\ are configured as $m_0=2$, $j_0=10$ and $T_0= 20$ for all six datasets.
% (recall that $m_0$, $j_0$ and $T_0$ are the three hyper-parameters for \deltagradl).
% and are included in Appendix \ref{appendix-sec: hyper}.

\begin{table}[h]
    \centering
    \small
    \caption{The hyper-parameters for each dataset}\label{Table: hyper_params}
    \vspace{-0.2cm}
    \begin{tabular}[!h]{|>{\arraybackslash}p{1.7cm}|>{\centering\arraybackslash}p{0.7cm}|>{\centering\arraybackslash}p{0.7cm}|>{\centering\arraybackslash}p{0.9cm}|>{\centering\arraybackslash}p{0.7cm}|>{\centering\arraybackslash}p{0.5cm}|>{\centering\arraybackslash}p{0.7cm}|} \hline
        \makecell{Dataset} &\mimic & \retina & \chexpert & \fashion & \fact & \twitter \\\hline
        Learning rate & 0.0005 & 0.001 & 0.02 &0.05 &0.005&0.01\\\hline
        L2 regularization & 0.05 & 0.05 & 0.05 &0.001 &0.01 &0.01\\ \hline
        \# of epochs & 150& 200 & 200 & 200& 150&400\\ \hline
        % \# of samples with ground truth & 80649 & 88703 & 43114 & 29323 & 514&74\\ \hline
    \end{tabular}
    % \caption{Caption}
\end{table}

% and 
% resulting transformed features are then used to train a logistic regression model through . 
% To train the logistic regression models, we run SGD with mini-batch size 1000,  and the . . 
% The hyper-parameters used for \sgd\ and \deltagrad\ are included in Appendix \ref{appendix-sec: hyper}.



\eat{However, as discussed in Section \ref{sec: method}, the strong convexity assumption on model type is only required for \deltagradg\ and \deltagradl, but not for \infl. }
% Also as mentioned above, since \infl\ is suitable for more general settings, 



\textbf{Sample selector setup} 
% Unless explicitly stated, 
We assume that the clean budget $B=100$, meaning that 100 training samples are cleaned in total.
% total number of training samples to be cleaned is 1000, which is also referred to as the cleaning budget. 
% As described in Section \ref{sec: intro}, there are two possible ways to select the 500 samples for cleaning. One is to leverage the {\em sample selector} to identify Top-500 influential training samples and
We further vary the number of samples to be cleaned at each round, i.e. the value of $b$. 

% Specifically, two different values of $b$ are used, i.e., 100 and 10.
% to show the benefit of using smaller $b$.
% and let them interact with the {\em Model constructor} after each batch to check whether they can stop early, 
% which means that this process needs to be 
% which is then repeated at most $\lceil\frac{1000}{b}\rceil$ times (recall that early stopping may occur). 
% Unless explicitly stated, 
% \infl\ is the default method in the {\em Sample selector} for evaluating the sample influence.
% (denoted as \cleanone) while the other one is to go through the loop \encircle{2} in Figure \ref{fig:pipeline} for multiple rounds, say, 10 rounds, by allowing the {\em Sample Selector} to provide a smaller set of the most influential samples, e.g. 50 of such samples, to the human annotators, and then letting the {\em Model Constructor} to update the models on the updated training dataset.  
% % is repeated for 10 rounds until the total cleaning budget is exhausted (denoted as \cleantwo). 
% Both of the two strategies will be compared in the experiments.
% Since the first round is regarded as the initialization step as introduced in Section \ref{sec: intro}, we only present the results for the last 9 rounds.

\textbf{Baseline against \infl} We compare \infl\ against several baseline methods that can also prioritize the most influential samples for label cleaning in the sample selector, including the original version of the influence function, i.e. Equation \eqref{eq: influence function} \cite{koh2017understanding} (denoted by \inflo), two active learning methods---least confidence based sampling method (denoted by \ac) and entropy based sampling method (denoted by \actwo) \cite{settles2009active}---and one noisy sample detection algorithm, \ou\ \cite{huang2019o2u}. Note that for fair comparison, Equation \eqref{eq: obj_function} is used for model training 
% when \infl\ or other baseline methods are 
no matter which method is used in the sample selector.
\eat{Equation \eqref{eq: prev_influence} \cite{zhang2018training} (denoted by \inflg) and \duti. 
Since solving the bi-level optimization problem in \duti\ is extremely expensive, %it is unreasonable to repeat this multiple times. 
we only run \duti\ once to identify the Top-100 influential training samples.}

\eat{Since active learning and noisy sample detection algorithms , they are also compared against \infl. Specifically, we consider two active learning methods, i.e., least confidence based sampling method (denoted by \ac) and entropy based sampling method (denoted by \actwo) \cite{settles2009active}, and two noisy sample detection algorithms, i.e., \ou\ \cite{huang2019o2u} and \tars\ \cite{dolatshah12cleaning}.}
% , in which the first one belongs to active learning algorithms while the latter two are recent efforts on detecting training samples with noisy labels.
% But note that 

Note that there also exist many other potential baseline methods, such as \duti\ \cite{zhang2018training} and \tars\ \cite{dolatshah12cleaning}. However, they are not applicable in the presence of either probabilistic labels or the regularization on uncleaned training samples. The comparison between \infl\ and those methods are included in the extended technical report \cite{wu2021chef}. 
\eat{For other baseline methods such as \ac, \actwo, \ou\ and \inflo, no modifications are made other than using Equation \eqref{eq: obj_function} for model training.}
% are not originally taken into considerations by .

\eat{Hence, we modify the methods to handle these scenarios or adjust the experimental set-up to create a fair comparison. For example, in Appendix \ref{appendix-sec: duti}, we present necessary modifications to \duti\ so that it can handle probabilistic labels. However, it is not straightforward to modify \duti\ for quantifying the effect of up-weighting the training samples after they are cleaned. We therefore only compare \duti\ against \infl\ when all the training samples are equally weighted (i.e. $\gamma=1$ in Equation \eqref{eq: obj_function}), which is presented in Appendix \ref{sec: exp_vary_weight}. Similarly, \tars\ is only applicable when the noisy labels are either 0 or 1 rather than probabilistic ones. Therefore, to compare \infl\ and \tars, we round the probabilistic labels 
% on the uncleaned samples 
to their nearest deterministic labels for a fair comparison (see Appendix \ref{sec: exp_tars} for details). For other baseline methods such as \ac, \actwo, \ou\ and \inflo, no modifications are made other than using Equation \eqref{eq: obj_function} for model training.}
% However, it is not straightforward to make such adaptations for all of those baseline approaches, such as \duti, which are discussed in details . 

% Note that \duti\ can automatically reason about the possibly cleaned labels, which can thus be served as the clean labels for the uncleaned samples (similar to \cleantwo). But for other baseline methods, cleaning the probabilistic labels totally rely on the human annotators' efforts and we employ majority vote to resolve the labeling conflicts from different (simulated or realistic) human annotators (similar to \cleanone).
% those methods are  \duti\ \cite{zhang2018training}, which is adapted to handle probabilistic labels (see 
% Appendix \ref{appendix-sec: duti} for details). However, 

\textbf{Baseline against \deltagradl\ and \deltagradg} Recall that \deltagradl\ incrementally updates the model after some training samples are cleaned.  We compare this with retraining the model from scratch (denoted as 
\retrain). 
We also compare the running time for selecting the influential training samples with and without \deltagradg. When \deltagradg\ is not used, it is denoted as \full.
% We also demonstrate the effectiveness of \deltagradg\ on picking up the influential training samples by comparing it against the way to reevaluate the influence of all uncleaned training samples (denoted as \full).
% To demonstrate the effectiveness of \deltagradg\ 
% % in reducing the overhead 
% on picking up the influential training samples, it is compared against the way to reevaluate the influence of all uncleaned training samples (denoted as \full).

% \textBF{Hyper-parameter settings} 
% But notice that applying \deltagrad\ or \retrain\ to update the model parameters may lead to the termination of the training process at different epochs. Therefore, for fair comparison of the running time for \deltagrad\ and \retrain, we run SGD for fixed number of epochs and record the running time of the two methods. After the training process is done. we apply the early stopping on the model parameters cached at each SGD epoch to determine the model parameters. 

% To incrementally update models for \mimic, \chexpert\ and \retina, those three parameters are determined as  respectively.




\eat{\begin{figure*}[h]
\includegraphics[width=2.0\columnwidth]{figures/incremental_time.eps}
\caption{Running time comparison between \deltagradg\ (green) and \full (yellow)}\label{fig:increm_time}
% \vspace{-0.35cm}
\end{figure*}}

\begin{figure}[ht]
\includegraphics[width=0.8\columnwidth, height=0.45\columnwidth]{figures/training_time_accuracy.png}
\caption{Comparison of running time between \deltagradl\ and \retrain}\label{fig:training_time}
% \vspace{-0.35cm}
\end{figure}

% \vspace{-0.5cm}
\subsection{Experimental design}\label{sec: exp_design}


% \begin{table}
%     \centering
%     \small
%     \caption{Comparison of the model prediction performance (F1 score) after 2000 training samples using \cleanone, \cleantwo\ and \cleanthree}\label{Table: prediction_strategy}\label{Table: strategy_compare}
%     \vspace{-0.2cm}
%     \begin{tabular}[!h]{|>{\arraybackslash}p{0.9cm}|>{\arraybackslash}p{1.75cm}|>{\centering\arraybackslash}p{1.45cm}>{\centering\arraybackslash}p{1.45cm}>{\centering\arraybackslash}p{1.45cm}|} \hline
%          \multicolumn{2}{|c|}{}&\mimic & \retina & \chexpert \\\hline
%          \multirow{4}{*}{\makecell{F1 score}}&Before cleaning& 0.7251$\pm$0.0217 & 0.7350$\pm$0.0037 & 0.5546$\pm$0.0149  \\\hhline{~----}
%         &\cleanone\ & 0.7412$\pm$0.0213 & 0.7733$\pm$0.0035&0.5658$\pm$0.0149 \\\hhline{~----}
%         &\cleantwo\ & \textBF{0.7414$\pm$0.0213} & \textBF{0.7737$\pm$0.0035}&\textBF{0.5660$\pm$0.0149}\\ \hhline{~----}
%         &\cleanthree\ & 0.7413$\pm$0.0213 & 0.7736$\pm$0.0035&0.5659$\pm$0.0149 \\ \hline
%         \multicolumn{2}{|c|}{\makecell{Average \# of correctly \\ suggested labels \\ (\cleantwo, out of 2000)}} & 1984.7 & 1988.3 &1953.0  \\\hline
%         \multicolumn{2}{|c|}{\makecell{Average \# of correctly \\ suggested labels \\ (\infl, out of 2000)}} & 1870.0 & 1905.7 & 1506.0 \\\hline
%     \end{tabular}
%     % \caption{Caption}
% \end{table}
\begin{table*}
    \centering
    \small
    \caption{Comparison of the model prediction performance (F1 score) after 100 training samples are cleaned}\label{Table: prediction_strategy}
    \vspace{-0.2cm}
    \begin{tabular}[!h]{>{\arraybackslash}p{1cm}||>{\arraybackslash}p{1cm}||>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.7cm}|>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{0.7cm}} \hline
    && \multicolumn{3}{c|}{b=100} & \multicolumn{8}{c}{b=10} \\ \hhline{~~-----------}
         & uncleaned&\cleanone\ & \cleantwo\ & \cleanthree\  & \inflo & \ac\ & \actwo\ & \ou & \cleanone\ & \cleantwo\ & \cleantwo\ + \deltagrad & \cleanthree\ \\\hline
        %  \multirow{}{*}{\makecell{F1 score}}&Before cleaning& 0.7251$\pm$0.0217 & 0.7350$\pm$0.0037 & 0.5546$\pm$0.0149  \\\hhline{~----}
        \mimic&0.6284 & 0.6292 & 0.6293 &0.6293&0.6283&0.6287&0.6287&0.1850&0.6292&\textBF{\underline{0.6293$\pm$0.0011}}&\textBF{0.6292$\pm$0.0005}&0.6292 \\
        \retina&0.5565&0.5580&\textBF{0.5582}&0.5581&0.5556&0.5568&0.5568&0.1314&0.5579&\textBF{0.5582$\pm$0.0003}&\textBF{\underline{0.5610$\pm$0.0010}}&0.5581\\ 
        \chexpert&0.5244& 0.5286&0.5297&0.5289&0.5246&0.5246&0.5246&0.5281&0.5287&\textBF{\underline{0.5300$\pm$0.0018}}&\textBF{0.5295$\pm$0.0030}&0.5291 \\ 
        \fashion&0.5140 & 0.5178&0.5177&0.5177&0.5143&0.5145&0.5145&0.5152      &0.5178&\textBF{0.5181$\pm$0.0131}&\textBF{\underline{0.5195$\pm$0.0144}}&0.5180 \\
        \fact& 0.6595 & 0.6601 & \textBF{0.6609} &0.6603&0.6596&0.6600&0.6600&0.6598&0.6601&\textBF{\underline{0.6609$\pm$0.0043}}&\textBF{\underline{0.6609$\pm$0.0065}}&0.6602 \\
        \twitter& 0.6485& 0.6594&0.6680&0.6594&0.6518&0.6515&0.6515&0.6490&0.6578&\textBF{\underline{0.6697$\pm$0.0058}}&\textBF{0.6597$\pm$0.0027}&0.6586 \\ \hline
        % \multicolumn{2}{|c|}{\makecell{Average \# of correctly \\ suggested labels \\ (\cleantwo, out of 2000)}} & 1984.7 & 1988.3 &1953.0  \\\hline
        % \multicolumn{2}{|c|}{\makecell{Average \# of correctly \\ suggested labels \\ (\infl, out of 2000)}} & 1870.0 & 1905.7 & 1506.0 \\\hline
    \end{tabular}
    % \caption{Caption}
\end{table*}

\eat{
\begin{table}
    \centering
    \small
    \caption{Comparison of the model prediction performance (F1 score) after 100 training samples are cleaned (CNN, b = 10)}\label{Table: strategy_compare_cnn0}
    \vspace{-0.2cm}
    \begin{tabular}[!h]{>{\arraybackslash}p{0.7cm}||>{\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{0.5cm}>{\centering\arraybackslash}p{0.5cm}>{\centering\arraybackslash}p{0.5cm}>{\centering\arraybackslash}p{0.5cm}>{\centering\arraybackslash}p{0.5cm}>{\centering\arraybackslash}p{0.5cm}>{\centering\arraybackslash}p{0.5cm}} \hline
    % && \multicolumn{3}{c|}{b=100} & \multicolumn{7}{c}{b=10}\\ \hhline{~~----------}
         & uncleaned & \cleanone & \cleantwo & \cleanthree & \inflo & \ac & \actwo & \ou \\\hline
        %  \multirow{}{*}{\makecell{F1 score}}&Before cleaning& 0.7251$\pm$0.0217 & 0.7350$\pm$0.0037 & 0.5546$\pm$0.0149  \\\hhline{~----}
        \mimic&0.8893&0.8893&\textBF{0.8908}&0.8904&0.8895&0.8895&0.8895&0.8873 \\
        \retina&0.5602&0.5596&\textBF{0.5645}&0.5607&0.5556&0.5574&0.5574&0.5608\\ 
        % \chexpert& \\
        % \fashion& \\
        \fact&0.7636&0.7553&\textBF{0.8063}&0.7654&0.7560&0.7566&0.7516&0.7739 \\
        \twitter&0.6783&0.6585&\textBF{0.6907}&0.6745&0.6642&0.6544&0.6610&0.6740 \\ \hline
        % \multicolumn{2}{|c|}{\makecell{Average \# of correctly \\ suggested labels \\ (\cleantwo, out of 2000)}} & 1984.7 & 1988.3 &1953.0  \\\hline
        % \multicolumn{2}{|c|}{\makecell{Average \# of correctly \\ suggested labels \\ (\infl, out of 2000)}} & 1870.0 & 1905.7 & 1506.0 \\\hline
    \end{tabular}
    % \caption{Caption}
\end{table}
}
% \begin{table*}
%     \centering
%     \small
%     \caption{Comparison of the model prediction performance (F1 score) after 1000 training samples are cleaned}\label{Table: prediction_strategy}\label{Table: strategy_compare}
%     \vspace{-0.2cm}
%     \begin{tabular}[!h]{>{\arraybackslash}p{1cm}||>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}|>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}>{\centering\arraybackslash}p{1.15cm}} \hline
%     & \multicolumn{3}{c|}{b=1000} & \multicolumn{8}{c}{b=20} \\ \hhline{~-----------}
%          &\infl\ (\cleanone)0 & \infl\ (\cleantwo)3 & \infl\ (\cleanthree)1 & \infl\ (\cleanone) & \infl\ (\cleantwo) & \infl\ (\cleanthree) & \inflg & \inflo & \duti & \ac& \ou \\\hline
%         %  \multirow{}{*}{\makecell{F1 score}}&Before cleaning& 0.7251$\pm$0.0217 & 0.7350$\pm$0.0037 & 0.5546$\pm$0.0149  \\\hhline{~----}
%         \mimic&0.895$\pm$0.015 & \textBF{0.897$\pm$0.015} & 0.896$\pm$0.015&0.895$\pm$0.015&0.897$\pm$0.015&0.896$\pm$0.015&&0.893$\pm$0.015&&0.895$\pm$0.015&0.895$\pm$0.015 \\\hline
%         \retina& & \textBF{0.714$\pm$0.013} & \textBF{0.777$\pm$0.035}&\textBF{0.560$\pm$0.019}&&&&&&&\\ \hline
%         \chexpert&& 0.741$\pm$0.021 & 0.736$\pm$0.005&0.659$\pm$0.049&&&&&&& \\ \hline
%         \fashion& & 0.743$\pm$0.013 & 0.736$\pm$0.005&0.565$\pm$0.049&&&&&&& \\ \hline
%         \fact& & 0.741$\pm$0.021 & 0.736$\pm$0.035&0.659$\pm$0.019&&&&&&& \\ \hline
%         \twitter& & 0.743$\pm$0.023 & 0.736$\pm$0.005&0.659$\pm$0.049&&&&&&& \\ \hline
%         % \multicolumn{2}{|c|}{\makecell{Average \# of correctly \\ suggested labels \\ (\cleantwo, out of 2000)}} & 1984.7 & 1988.3 &1953.0  \\\hline
%         % \multicolumn{2}{|c|}{\makecell{Average \# of correctly \\ suggested labels \\ (\infl, out of 2000)}} & 1870.0 & 1905.7 & 1506.0 \\\hline
%     \end{tabular}
%     % \caption{Caption}
% \end{table*}



\eat{
\begin{table}
\centering
\small
\caption{The comparison of the prediction performance (F1 score) after 2000 training samples are cleaned}\label{Table: prediction_perf}
\vspace{-0.2cm}
\begin{tabular}[!h]{|>{\arraybackslash}p{1.3cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.3cm}|>{\centering\arraybackslash}p{1.3cm}|>{\centering\arraybackslash}p{1.3cm}|} \hline
%dataset
 \multicolumn{2}{|c|}{}&\mimic&\retina&\chexpert \\ \hhline{-----}
% & RMSE & MAE& RMSE & MAE& RMSE & MAE\\ \hline
\multirow{6}{*}{\makecell{F1 score}}&Before cleaning& 90.74$\pm$0.01 & 84.39$\pm$0.01 & 71.51$\pm$0.06  \\\hhline{~----}
% &\infl\ (\cleanone) & \textbf{93.80$\pm$1.17} &  \textbf{91.55$\pm$0.24} & \textbf{62.46$\pm$1.46}\\ \hhline{~----}
&\inflo & 91.77$\pm$0.01 & 85.24$\pm$0.01 & 73.51$\pm$0.06 \\
&\inflg & 91.15$\pm$0.01 & 84.78$\pm$0.01 & 71.08$\pm$0.06 \\
&\duti & 93.10$\pm$0.01&89.18$\pm$0.01 & 71.51$\pm$0.06\\
&\infl & \textbf{93.92$\pm$0.01} & \textbf{89.14$\pm$0.01} & \textbf{78.78$\pm$0.05} \\\hhline{~----}
&\infl\ + \deltagradl & \textbf{93.92$\pm$0.01} & \textbf{89.14$\pm$0.01} & \textbf{78.78$\pm$0.05} \\\hline
% \lstm & 1.0587$\pm$0.0091 & 0.8203$\pm$0.0106 & 0.6340$\pm$0.0098\\
% \dmm & 0.9852$\pm$0.0025 & 0.7510$\pm$0.0057 & 0.6068$\pm$0.0092\\
% \xgboost & 0.9900$\pm$0.0002 &0.7209$\pm$0.0003  & 0.8664$\pm$0.0011 \\
% \grui & 1.0322$\pm$0.0069 & 0.8256$\pm$0.0074 & 0.9491$\pm$0.0046 \\
% \grud & 1.0495$\pm$0.0068 & 0.8502$\pm$0.0069 & 0.9695$\pm$0.0089 \\
% IPN & 0.9888$\pm$0.0025 & 0.7856$\pm$0.0039 & 0.6097$\pm$0.0066 \\
% \lgnet & 0.9590$\pm$0.0033 & 0.7093$\pm$0.0033 & 0.5883$\pm$0.0071 \\ 
% \lode & 0.9315$\pm$0.0034 & 0.7325$\pm$0.0035 & 0.6171$\pm$0.0056 \\\hline
% \ourmethod-L & \underline{0.9143$\pm$0.0025} & \underline{0.7089$\pm$0.0037} \\
% \ourmethod-O & \textbf{0.9003$\pm$0.0015} & \textbf{0.6876$\pm$0.0027} & \textbf{0.4983$\pm$0.0053} \\ \hline
\end{tabular}
%\vspace*{-0.2cm}
\end{table}
}

% \begin{table}
% \centering
% \small
% \caption{Comparison of the prediction performance (F1 score) after 2000 training samples are cleaned}\label{Table: prediction_perf}
% \vspace{-0.2cm}
% \begin{tabular}[!h]{|>{\centering\arraybackslash}p{2.2cm}|>{\centering\arraybackslash}p{1.45cm}>{\centering\arraybackslash}p{1.45cm}>{\centering\arraybackslash}p{1.45cm}|} \hline
% %dataset
%  Methods &\mimic&\retina&\chexpert \\ \hhline{----}
% % & RMSE & MAE& RMSE & MAE& RMSE & MAE\\ \hline
% % \multirow{6}{*}{\makecell{Prediction\\ accuracy (\%)}}&Before cleaning& 90.74$\pm$0.01 & 84.39$\pm$0.01 & 71.51$\pm$0.06  \\\hhline{~----}
% % &\infl\ (\cleanone) & \textbf{93.80$\pm$1.17} &  \textbf{91.55$\pm$0.24} & \textbf{62.46$\pm$1.46}\\ \hhline{~----}
% \inflo & 0.7412$\pm$0.0213 & 0.7732$\pm$0.0035 & \textBF{0.5706$\pm$0.0149} \\
% \inflg & 0.7288$\pm$0.0216 & 0.7437$\pm$0.0037 & 0.5508$\pm$0.0150 \\
% \duti & 0.7244$\pm$0.0217&0.7376$\pm$0.0037 & 0.5503$\pm$0.0150\\\hline
% \infl & \textBF{0.7414$\pm$0.0213} & \textBF{0.7737$\pm$0.0035}&0.5660$\pm$0.0149 \\\hline
% \makecell{\infl\ + \deltagradl} & \textBF{0.7416$\pm$0.0213} & \textBF{0.7746$\pm$0.0035} & 0.5650$\pm$0.0150 \\\hline
% % \lstm & 1.0587$\pm$0.0091 & 0.8203$\pm$0.0106 & 0.6340$\pm$0.0098\\
% % \dmm & 0.9852$\pm$0.0025 & 0.7510$\pm$0.0057 & 0.6068$\pm$0.0092\\
% % \xgboost & 0.9900$\pm$0.0002 &0.7209$\pm$0.0003  & 0.8664$\pm$0.0011 \\
% % \grui & 1.0322$\pm$0.0069 & 0.8256$\pm$0.0074 & 0.9491$\pm$0.0046 \\
% % \grud & 1.0495$\pm$0.0068 & 0.8502$\pm$0.0069 & 0.9695$\pm$0.0089 \\
% % IPN & 0.9888$\pm$0.0025 & 0.7856$\pm$0.0039 & 0.6097$\pm$0.0066 \\
% % \lgnet & 0.9590$\pm$0.0033 & 0.7093$\pm$0.0033 & 0.5883$\pm$0.0071 \\ 
% % \lode & 0.9315$\pm$0.0034 & 0.7325$\pm$0.0035 & 0.6171$\pm$0.0056 \\\hline
% % \ourmethod-L & \underline{0.9143$\pm$0.0025} & \underline{0.7089$\pm$0.0037} \\
% % \ourmethod-O & \textbf{0.9003$\pm$0.0015} & \textbf{0.6876$\pm$0.0027} & \textbf{0.4983$\pm$0.0053} \\ \hline
% \end{tabular}
% %\vspace*{-0.2cm}
% \end{table}


In this section, we design the following three experiments:

\eat{In the experiments, we answer the following questions:
\begin{enumerate}[label=\textbf{Q\arabic*}]
    % \item: Can the model performance be guaranteed when the labels suggested by \infl\ are regarded as one additional labeler? \label{q1}
    \item: Can \infl\  beat other baseline methods in terms of the performance of the final models, in particular, if labels suggested by \infl\ are regarded as one additional labeler? \label{q2}
    % \vspace{-0.3cm}
    \item: Will \deltagradg\ speed up the selection of influential samples in the sample selector phase? \label{q3}
    \item: Will \deltagradl\ accelerate 
    % updating the model in 
    the model constructor phase without degrading the model performance? \label{q4}
\end{enumerate}

% \vspace{-0.3cm}
To answer these questions, we designed the following experiments:}

% \begin{table*}[h]
% \centering
% \small
% \caption{Running time comparison between \deltagradg\ and \full\ in the last cleaning round}\label{Table: running_time_last}
% \vspace{-0.2cm}
% \begin{tabular}[!h]{>{\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{2.6cm}|>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{2.6cm}|>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{2.6cm}} \hline
% %dataset
% \multirow{2}{*}{Iteration} &\multicolumn{2}{c|}{\mimic}&\multicolumn{2}{c|}{\retina}&\multicolumn{2}{c}{\chexpert} \\ \hhline{~------}
% & \full\ & \deltagradg\ & \full\ & \deltagradg\ & \full\ & \deltagradg\ \\ \hline
% $\text{Time}_{inf}$ (s) & 43.330$\pm$0.498 & \textbf{2.772$\pm$0.032 \textcolor{red}{(15.6x)}} & 14.528$\pm$0.634 & \textbf{1.358$\pm$0.041 \textcolor{red}{(10.7x)}} & 14.238$\pm$0.223 & \textbf{1.255$\pm$0.028 \textcolor{red}{(11.3x)}} \\
% $\text{Time}_{grad}$ (s) & 39.197$\pm$0.659 & \textbf{0.168$\pm$0.026 \textcolor{red}{(233.3x)}} & 12.998$\pm$0.609  & \textbf{0.213$\pm$0.026 \textcolor{red}{(61.0x)}} & 12.815$\pm$0.219 & \textbf{0.076$\pm$0.006 \textcolor{red}{(168.6x)}}\\
% count & 78487 & \textbf{339.600$\pm$53.758} & 31614 & \textbf{391.800$\pm$44.096} & 38629 & \textbf{146.000$\pm$14.366} \\\hline
% \end{tabular}
% %\vspace*{-0.2cm}
% \end{table*}

\eat{
\begin{table*}[h]
\centering
\small
\caption{Running time comparison between \deltagradg\ and \full\ in the last cleaning round}\label{Table: running_time_last}
\vspace{-0.2cm}
\begin{tabular}[!h]{>{\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{2.6cm}|>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{2.6cm}|>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{2.6cm}} \hline
%dataset
\multirow{2}{*}{} &\multicolumn{2}{c|}{$\text{Time}_{inf}$ (s)}&\multicolumn{2}{c|}{$\text{Time}_{grad}$ (s)}&\multicolumn{2}{c}{count} \\ \hhline{~------}
& \full\ & \deltagradg\ & \full\ & \deltagradg\ & \full\ & \deltagradg\ \\ \hline
\mimic  & 43.330$\pm$0.498 & \textbf{2.772$\pm$0.032 \textcolor{red}{(15.6x)}} &39.197$\pm$0.659  & \textbf{0.168$\pm$0.026 \textcolor{red}{(233.3x)}} & 78487 & \textbf{339.600$\pm$53.758} \\
\retina &14.528$\pm$0.634  & \textbf{1.358$\pm$0.041 \textcolor{red}{(10.7x)}} & 12.998$\pm$0.609  &  \textbf{0.213$\pm$0.026 \textcolor{red}{(61.0x)}} & 31614 & \textbf{391.800$\pm$44.096}\\
\chexpert &14.238$\pm$0.223  & \textbf{1.255$\pm$0.028 \textcolor{red}{(11.3x)}} &12.815$\pm$0.219 & \textbf{0.076$\pm$0.006 \textcolor{red}{(168.6x)}} & 38629 & \textbf{146.000$\pm$14.366} \\
\fashion &127.021$\pm$3.549 &\textbf{11.446$\pm$0.598 \textcolor{red}{(11.1x)}} &115.483$\pm$3.313 & \textbf{0.930$\pm$0.074 \textcolor{red}{(124.2x)}}& 29301 & \textbf{203.250$\pm$1.422}  \\
\fact &156.307$\pm$4.023 &\textbf{8.969$\pm$0.755 \textcolor{red}{(17.4x)}} &125.84$\pm$5.972 & \textbf{0.707$\pm$0.037 \textcolor{red}{(178.0x)}} &38176 &\textbf{204.667$\pm$1.155}  \\
\twitter &55.676$\pm$2.342 &\textbf{8.470$\pm$0.437 \textcolor{red}{(6.6x)}} &37.388$\pm$1.121 &\textbf{0.784$\pm$0.042 \textcolor{red}{(47.7x)}} &11606  &\textbf{233.889$\pm$8.818} \\\hline
\end{tabular}
%\vspace*{-0.2cm}
\end{table*}
}


\begin{table}[h]
\centering
\small
\caption{Running time of \deltagradg\ and \full}\label{Table: running_time_last}
\vspace{-0.2cm}
\begin{tabular}[!h]{>{\arraybackslash}p{0.9cm}||>{\centering\arraybackslash}p{0.8cm}>{\centering\arraybackslash}p{2.3cm}|>{\centering\arraybackslash}p{0.8cm}>{\centering\arraybackslash}p{2.2cm}} \hline
%dataset
\multirow{2}{*}{} &\multicolumn{2}{c|}{$\text{Time}_{inf}$ (s)}&\multicolumn{2}{c}{$\text{Time}_{grad}$ (s)} \\ \hhline{~----}
& \full\ & \deltagradg\ & \full\ & \deltagradg\ \\ \hline
\mimic  & 151.4$\pm$0.5 & \textbf{2.77$\pm$0.03 \textcolor{red}{(54.7x)}} &145.4$\pm$0.7  & \textbf{0.17$\pm$0.03 \textcolor{red}{(855x)}} \\
\retina &74.0$\pm$0.6  & \textbf{1.36$\pm$0.04 \textcolor{red}{(54.4x)}} & 70.8$\pm$0.6  &  \textbf{0.21$\pm$0.03 \textcolor{red}{(337x)}} \\
\chexpert &72.5$\pm$0.2  & \textbf{17.9$\pm$1.9 \textcolor{red}{(4.1x)}} &69.3$\pm$0.2 & \textbf{14.7$\pm$1.5 \textcolor{red}{(4.7x)}} \\
\fashion &66.4$\pm$3.6 &\textbf{8.7$\pm$0.6 \textcolor{red}{(7.6x)}} &57.1$\pm$3.3 & \textbf{0.81$\pm$0.07 \textcolor{red}{(70.5x)}}\\
\fact &73.8$\pm$4.0 &\textbf{6.1$\pm$0.8 \textcolor{red}{(12.1x)}} &72.5$\pm$6.0 & \textbf{4.7$\pm$0.1 \textcolor{red}{(15.4x)}}  \\
\twitter &33.1$\pm$2.3 &\textbf{14.1$\pm$0.4 \textcolor{red}{(2.3x)}} &30.2$\pm$1.1 &\textbf{12.7$\pm$0.1 \textcolor{red}{(2.4x)}} \\ \hline
\end{tabular}
%\vspace*{-0.2cm}
\end{table}


\textbf{Exp1} 
%As discussed above, when \infl\ is used in the {\em Sample selector}, we can choose to aggregate the suggested labels by \infl\ and the cleaned labels by two simulated human annotators as the final cleaned labels for the most influential training samples. 
% To demonstrate the performance advantage of \infl, as mentioned above, 
In this experiment, we compared the model prediction performance after \infl\ and other baseline methods (including \inflo, \ac, \actwo, \ou) are applied to select 100 training samples for cleaning. Recall that there are three different strategies that \infl\ can use to provide cleaned labels and their performance is compared. 
To show the benefit of using a smaller batch size $b$, we choose two different values for $b$, i.e. 100 and 10. 
% There are three different strategies to provide clean labels  \cleantwo\ (majority vote of suggested label by \infl\ and two human annotators), we compare it against the following two alternatives in terms of the model prediction performance after the cleaning process is done: 1) \cleanone\ (majority vote of labels from three human annotators); and 2) \cleanthree\ (using the true label). 
Since the ground-truth labels are available for all samples in \cleanset, we count how many of them match the labels suggested by \infl.
% \ are with respect to the ground truth for those datasets, 
% Note that the true labels are not available in practice, but can be used for our experiments. We also investigated how many cleaned labels by \infl\ and \cleanone\ match the ground truth labels, 
% which can further demonstrate whether it is reasonable to regard \infl\ as an independent labeler. 


% (see Appendix \ref{sec: exp_supple}).
% As mentioned above, since $\gamma$ is not zero in Equation \eqref{eq: our_influence} the comparison between \infl\ and \duti, \inflg\ and \tars\ are included in the Appendix.
% methods, i.e. using the cleaned labels by three simulated human annotators (denoted as \cleantwo) without referencing the cleaning 
% the same number of training samples through \cleantwo\ can lead to better model performance than \cleanone, we implemented \infl\ in the sample selector and let the sample selector provide the most influential training samples to the human annotators through \cleanone\ and \cleantwo\ respectively. After the cleaning process is done, we compared the prediction performance of the resulting models produced by those two strategies.

\eat{\textbf{Exp2} The purpose of this experiment is to evaluate the model prediction performance when \infl\ is used in the {\em Sample selector} to evaluate the training sample influence, which is compared against two other versions of influence functions, e.g., Equation \eqref{eq: prev_influence} (denoted by \inflg\ \cite{zhang2018training}) and Equation \eqref{eq: influence function} (denoted by \inflo\ \cite{koh2017understanding}). 
Since those versions of influence functions cannot suggest cleaned labels, \cleanone\ is used to aggregate the cleaned labels by three simulated human annotators. 
% For all of these variants, the prediction performance is evaluated after the human annotators clean the uncertain labels for 10 iterations with 50 training samples to be cleaned at each iteration. 
We also compare \infl\ against }
%  , and \cleantwo\ is used to produce the cleaned labels.
% for providing all the influential training samples once with \duti\ implemented in the sample selector. 
% In this experiment, we are primarily interested in the prediction performance of the approaches listed above. 
\eat{We also investigated how many suggested deterministic labels by \infl\ can match the ones cleaned by the human annotators, i.e., the originally deterministic labels as described in Section \ref{sec: exp_setup}. This is also crucial since the sample influence calculated by \infl\ depends on how the uncertain labels are updated. Therefore, the mismatch between the suggested labels and the human annotated labels may lead to inaccurate estimations of the training sample influence. Consequently, the training samples selected for cleaning may not be optimal, thus eventually degrading the model performance.}
% DUTI from \cite{zhang2018training}
% Influence function from \cite{zhang2018training}
% influence function from \cite{koh2017understanding}
% our method; our method clean multiple times

\textbf{Exp2} \eat{Recall that \deltagradg\ can be coupled with \infl\ to 
% reduce the time overhead of identifying the most influential training samples by 
filter out most of the uninfluential samples early.  % without evaluating their influence. 
% To investigate whether this can reduce the time overhead of the sample selector, 
Therefore, }
This experiment compares the running time of selecting the Top-$b$ (with $b=10$) influential training samples (denoted $\text{Time}_{inf}$) with and without using \deltagradg\ at each round in the {\em Sample selector}  phase. 
\eat{When \deltagradg\ is not used, it means that the influence of {\em all} training samples are always re-evaluated, which is denoted as \full.}
% Same as \textbf{Exp1} and \textbf{Exp2}, both of those two approaches are implemented in the {\em Sample selector} to evaluate the influence by using Equation \eqref{eq: our_influence} for all or parts of the training samples and select the Top-50 influential training samples among them, which is repeated for 10 times. 
Recall that the most time-consuming step to evaluate Equation \eqref{eq: our_influence} is to compute the class-wise gradients for each sample and the sample-wise gradients.
% when we evaluate the training sample influence with \infl\ (i.e. Equation \eqref{eq: our_influence}), computing the class-wise gradients for each sample is the most time-consuming step. 
Therefore, its running time 
% of this step 
(denoted as $\text{Time}_{grad}$) is also recorded. For \deltagradg, the time to compute the bounds in Theorem \ref{theorem: bound_influence} is also included in $\text{Time}_{inf}$.
% We also break down $\text{Time}_{inf}$ by recording  and other steps (denoted as $\text{Time}_{other}$).  
% Therefore, in addition to $\text{Time}_{inf}$, 
% % To demonstrate how \deltagradg\ can accelerate this step, 
% we also record the running time to compute the sample-wise gradients  and other components of Equation \eqref{eq: our_influence}  respectively for both \deltagradg\ and \full. 
% As a result, $\text{Time}_{inf}$ is composed of $\text{Time}_{grad}$ and the running time on other steps for evaluating Equation \eqref{eq: our_influence} (denoted as $\text{Time}_{other}$). 

\textbf{Exp3} 
% After the labels of the influential training samples are cleaned, the next step refreshes the model parameters ({\em Model constructor}).
% after the human annotators clean the labels of the influential training samples. 
% The model parameters can be updated either by retraining from scratch (denoted \retrain) or by applying \deltagradl. 
The main goal of this experiment is to explore the difference in running time between \retrain\ and \deltagradl\ for updating the model parameters in the {\em Model constructor} phase.
% how much speed-up that  can achieve in  with respect to the way to retrain from scratch  when some uncertain training labels are cleaned at each iteration. 
% Specifically, at each iteration of the loop \encircle{2}, we follow the experimental designs from \cite{wu2020deltagrad} to compare the running time of \deltagradl\ and \retrain\ as well as the differences of the models produced by those two approaches after the human annotators clean the {\em same} set of training labels. 
In addition,  the model parameters produced by \deltagradl\ and \retrain\ are not exactly the same 
%the theoretical analysis provided 
\cite{wu2020deltagrad}, which could lead to different influence values for each training sample and
% when Equation \eqref{eq: our_influence} is calculated for each training sample, 
thus produce different models
% generate different sets of influential training samples 
in subsequent cleaning rounds.
% for \deltagradl\ and \retrain\ in the Sample Selector. 
% Note that those differences can also be accumulated in the following cleaning rounds in the loop \encircle{2}. 
Therefore, we also explore whether such differences
% This means that the differences of the models constructed by \deltagradl\ and \retrain\ may lead to variations on the influence measures and the subsequent selected influential training samples, 
produce divergent prediction performance for \deltagradl\ and \retrain.

\begin{figure}[h]
  \centering
  \begin{subfigure}{.45\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/visualization.png}
    \caption{\twitter}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.45\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/visualization_fashion.png}
    \caption{\fashion}
  \end{subfigure}%
%   \hfill
%   \begin{subfigure}{.3\columnwidth}
%     \centering
%     \includegraphics[width=\linewidth]{example-image-c}
%     \caption{Level 3}
%   \end{subfigure}
  \caption{Visualization of the validation samples, test samples and the most influential training sample $S$ (`+', `-' and `X' denote the positive ground-truth samples, negative ground-truth samples and the sample $S$ respectively)}\label{fig:twitter_visual}
\end{figure}
% As Figure \ref{fig:training_time}, the models produced by \deltagradl\ and \retrain\ always have statistically the same prediction performance. To further explore
% after those differences on models and influence measures are accumulated for several iterations in the loop \encircle{2}.  


% Same as \textbf{Exp1} and \textbf{Exp2}, we go through the loop \encircle{2} for 10 times. 



% \xgboost & 0.9900$\pm$0.0002 &0.7209$\pm$0.0003  & 0.8664$\pm$0.0011 & 0.7816$\pm$0.0010  & 0.8841$\pm$0.0106 & 0.7580$\pm$0.0102\\
% \grui & 1.0322$\pm$0.0069 & 0.8256$\pm$0.0074 & 0.9491$\pm$0.0046 & 0.7764$\pm$0.0049 & 0.8233$\pm$0.0333 & 0.5925$\pm$0.0364\\
% \grud & 1.0495$\pm$0.0068 & 0.8502$\pm$0.0069 & 0.9695$\pm$0.0089 & 0.7912$\pm$0.0087 & 0.7268$\pm$0.0254 & 0.5051$\pm$0.0228\\
% IPN & 0.9888$\pm$0.0025 & 0.7856$\pm$0.0039 & 0.6097$\pm$0.0066 & 0.4204$\pm$0.0089 & 0.7207$\pm$0.0313 & 0.4834$\pm$0.0229\\
% \lgnet & 0.9590$\pm$0.0033 & 0.7093$\pm$0.0033 & 0.5883$\pm$0.0071 & \underline{0.3841$\pm$0.0063} & 0.7346$\pm$0.0272 & 0.5181$\pm$0.0218\\ 
% \lode & 0.9315$\pm$0.0034 & 0.7325$\pm$0.0035 & 0.6171$\pm$0.0056 & 0.4216$\pm$0.0038 & 0.8226$\pm$0.0387 & 0.5834$\pm$0.0331\\\hline
% \ourmethod-L & \underline{0.9143$\pm$0.0025} & \underline{0.7089$\pm$0.0037} & \underline{0.5426$\pm$0.0066} & 0.3848$\pm$0.0047 & \underline{0.6975$\pm$0.0224} & \underline{0.4748$\pm$0.0162}\\
% \ourmethod-O & \textbf{0.9003$\pm$0.0015} & \textbf{0.6876$\pm$0.0027} & \textbf{0.4983$\pm$0.0053} & \textbf{0.3367$\pm$0.0059} & \textbf{0.6835$\pm$0.0276} & \textbf{0.4646$\pm$0.0213}\\ \hline


\subsection{Experimental results}\label{sec: exp_res}

\textbf{Exp1} Experimental results 
%of \textbf{Exp1} 
are given in Table \ref{Table: prediction_strategy}\footnote{
% Except \cleantwo, only the averaged F1 scores are given. 
Due to space limit, the error bars of most F1 scores are included in the extended technical report \cite{wu2021chef}}.
% which includes averaged model performance. 
We observe that with fixed $b$, e.g., 10, \cleantwo\ performs best across almost all datasets. Recall that \cleantwo\ 
% evaluates the training sample influence with Equation \eqref{eq: our_influence} and
uses the derived labels produced by \infl\ as the cleaned labels without additional human annotated labels. Due to its superior performance, % than the other two strategies, i.e. \cleanone\ and \cleantwo, 
especially on \crowdset,
% Since \cleantwo\ performs significantly better than \cleanone\ and \cleanthree\ where the human annotations are involved, 
this implies that the quality of the labels provided by \infl\ could actually be better than that of the human annotated labels.
% able to provide more reasonable labels than human annotators in boosting the prediction performance. 

To further understand 
% the reason behind 
this phenomenon, we compared the labels suggested by \infl\ against their ground-truth labels for \cleanset.  It turns out that over 70\% are equivalent (89 for \retina, 79 for \chexpert\ and 95 for \mimic). Note that even the ground-truth labels of these three datasets are not 100\% accurate. In the \chexpert\ dataset, for example, the ground-truth labels are generated through an automate labeling tool rather than being labeled by human annotators,
% ,  is employed to extract the labels from the text files for all the samples , 
thereby leading to possible labeling errors. Those erroneous labels may not match the labels provided by \infl, thus leading to worse model performance (see the performance difference between \cleanone\ and \cleantwo\ for \chexpert\ dataset). 
% Since simply using the suggested labels by \infl, i.e. \cleantwo, leads to better performance than purely using the human annotated labels, i.e. \cleanthree, we can  Consequently, \infl\ is likely to provide better labels than the ground-truth labels, thus leading to better model performance.
% why \cleantwo\ is able to suggest much better labels than \cleanthree\ and \cleanone, 

However, the above comparison could not be done for \crowdset\ due to the lack of ground-truth labels. We therefore investigate the relationship between the samples with ground-truth labels and the influential samples identified by \infl. Specifically, 
we use t-SNE \cite{van2008visualizing} to visualize the 
% validation set and the test set 
samples with ground-truth labels
for the \twitter\ and \fashion\ datasets after the feature transformation using the pre-trained models (see Figure \ref{fig:twitter_visual}). As described in Section \ref{sec: exp_setup}, those samples belong to validation or test set.
% To distinguish positive and negative samples from those two sets, we use blue circle and red plus symbol respectively. 
In addition, in this figure, we indicate the position of the most influential training sample $S$ identified by \infl.
% , which is denoted by green cross mark symbol.
% to highlight the position of the sample $S$.
As this figure indicates, the sample $S$ is proximal to the samples with negative ground-truth labels for the \twitter\ dataset (positive for the \fashion\ dataset). To guarantee the accurate predictions on those nearby ground-truth samples, it is therefore reasonable to label $S$ as negative (positive for \fashion\ dataset), which matches the labels provided by \infl\ but differs from ones given by the human annotators. This indicates the high quality of the labels given by \infl. 
% at giving labels to  We also observe similar results for \fact\ dataset. Note that no human annotated labels are used in \cleantwo, which thus indicates that \cleantwo\ can not only lead to better model performance, but also reduce the human annotation cost. 
Thus, when high-quality human labelers are unavailable, \infl\ can be an alternative labeler for reducing the labeling cost without harming the labeling quality.%, which answers \textbf{Q1}.

Table \ref{Table: prediction_strategy} also exhibits the benefit of using smaller batch sizes $b$ since it results in better model performance when \infl, especially \cleantwo, is used for some datasets (e.g, see its model performance comparison between $b=100$ and $b=10$ for \twitter\ dataset in Table \ref{Table: prediction_strategy}). 
%(see the performance difference of \infl\ with varied $b$ in Table \ref{Table: prediction_strategy}).
% (except \retina\ dataset\footnote{Despite the lower F1-score when $b=100$ for \retina\ dataset, we observe that the loss on the test dataset with $b=100$ is still smaller than that with $b=1000$})
Intuitively, \infl\ only quantifies the influence of 
% updating the label and the weight of 
cleaning {\em single} training sample rather than multiple ones. Therefore, the larger $b$ is, the more likely that \infl\ selects a sub-optimal set of $b$ samples for cleaning. Ideally, $b$ should be one, meaning that one training sample is cleaned at each round. However, this can inevitably increase 
the number of rounds and thus 
the overall overhead. Intuitively speaking, a medium size of $b$ should be a reasonable choice to balance the model performance and the total running time, which is empirically demonstrated in \cite{wu2021chef}.
% We also empirically explored how to choose an appropriate $b$ to balance the model performance and the total running time in \cite{wu2021chef}.
% demonstrate this point, we investigate some training samples that \infl\  In addition, 
\eat{thus indicating the advantage of \infl\ on identifying more valuable training samples for cleaning shows that the model prediction performance using \cleanone, \cleantwo\ and \cleanthree\ are almost the same, and significantly better than the model performance prior to the cleaning process. 
% It is also worth noting that \cleanone\ slightly outperforms \cleantwo\ in \chexpert. 
According to the last two rows of Table \ref{Table: strategy_compare}, 
the closeness in model performance among the three strategies can be further justified by 1) the almost equivalent labels provided by the three strategies (second to last row); 2) at least 75\% overlaps between the suggested labels by \infl\ and the ground truth (last row), which is still smaller than the worst human annotator error (30\% according to \cite{brady2017error}). This result indicates that using \infl\ as one ``annotator'' is feasible, and can save the cost of having one additional human annotator. These experimental results help answer \ref{q1}.}
% . use of \cleantwo\ can significantly enhance the model prediction performance with respect to \cleanone\ in all the three datasets. 
% The intuitive explanation is that for \cleantwo, as \cleantwo\ proceeds, the selections of the  
% This thus justifies the performance advantage of iteratively cleaning label uncertainties via \cleantwo\ and addresses \ref{q1}. 
% Recall that for \cleantwo, it involves interactions between the human annotators, the sample selector and the model constructor for multiple rounds. Therefore, the remaining concern would be how to reduce the time overhead of such iterative process. 

% \begin{figure}[h]
%   \centering
%   \subfigure[random caption 1]{\includegraphics[scale=0.45]{figures/visualization.eps}}
%   \subfigure[random caption 2]{\includegraphics[scale=0.45]{figures/visualization_fashion.eps}}
% \end{figure}

% \begin{figure}[h]
% \includegraphics[width=0.5\columnwidth, height=0.45\columnwidth]{figures/visualization.eps}
% \caption{Visualization of the validation samples, test samples and the most influential training sample}\label{fig:twitter_visual}
% % \vspace{-0.35cm}
% \end{figure}



\eat{\textbf{Exp2} Experimental results are given in Table \ref{Table: prediction_perf} (ignore the last row for now), which  address \ref{q2}.
% First of all, we observe that applying different variants of the influence functions and \duti\ can improve the model prediction performance with respect to initial model performance (see the second to the fifth row VS the first row).
% is included in the second row to the fifth row of . 
% In addition, 
We observe that \infl\ can beat other variants of the influence functions in terms of the model prediction performance in \mimic\ and \retina, and performs slightly worse than \inflo\ in \chexpert. 
However, for \inflo, the slight performance gain comes at the cost of one additional human annotator.
%of \inflo\ requires one more human annotators with respect to \infl. 
As a result, \infl\ may be preferable due to its ability to balance cost and performance. This justifies the feasibility of explicitly including the label updates in \infl\ (i.e. $\delta_y$ in Equation \eqref{eq: our_influence}).   
\eat{We can further demonstrate that the performance advantage of \infl\ is due to the {\em near optimal} selections of the Top-2000 influential training samples. This is because as the last row of Table \ref{Table: prediction_perf} indicates, the suggested deterministic labels by \infl\ match the ground truth on most of the training samples, meaning that their influence calculated by Equation \eqref{eq: our_influence} is reasonable.}
% in terms of the model prediction performance after the same number of training samples are cleaned, 
% This is because 1) as discussed in Section \ref{sec: influence-l}, \infl\ determines the influence of a training sample with uncertain labels by {\em straightforwardly} estimating how updating its uncertain label to some deterministic one improves the prediction performance; 2) the suggested labels by \infl\ for the selected influential samples are mostly correct (see the last row of Table \ref{Table: prediction_perf}). 
Furthermore, it is worth noting that \infl\ even outperforms \duti. 
Based on our observations in the experiments, this phenomenon might be due to the difficulty in {\em exactly} solving the bi-optimization problem in \duti, thus producing sub-optimal selections of the influential training samples.
% by \duti\ may hurt the model performance. 
% This thus demonstrates that \infl\ is able to provide the training samples that are more likely to boost the model prediction performance after their label uncertainties are fixed.  Plus, we can observe that the prediction performance of \infl\ and \duti\ are pretty close. 
}






\textbf{Exp2} In this experiment, we compare the running time of \deltagradg\ and \full\ in selecting the Top-10 influential training samples ($\text{Time}_{inf}$) at each cleaning round of the loop \encircle{2} (with $b=10$). Due to space, we only include results for the last round in Table \ref{Table: running_time_last}, which are similar to results in other rounds.
% and the breakdown of this running time, i.e., $\text{Time}_{grad}$ and $\text{Time}_{other}$ included in Figure \ref{fig:increm_time}, which excludes the results of the first cleaning round (i.e, the initialization step)
% for each cleaning round in the loop \encircle{2}. 
% in which we exclude the results of the first round . 
As Table \ref{Table: running_time_last} indicates,  \deltagradg\ is up to 54.7x faster than \full,
% \ in identifying the 1000 most influential training samples, 
which is due to the significantly decreased overhead of computing the class-wise gradients for each sample (i.e. $\text{Time}_{grad}$) when \deltagradg\ is used. To further illustrate this point, we 
% include more detailed results of the last cleaning round in Table \ref{Table: running_time_last} for \deltagradg\ and \full. Those experimental results are comprised of $\text{Time}_{inf}$, $\text{Time}_{grad}$ and 
also record the number of candidate influential training samples whose influence values are explicitly evaluated with and without using \deltagradg.
% which indicates that is in the last two columns of Table \ref{Table: running_time_last}. 
The result indicates that due to the early removal of uninfluential training samples using \deltagradg, we only need to evaluate the influence of a small portion of training samples, thus reducing $\text{Time}_{grad}$ by up to two orders of magnitude and thereby significantly reducing the total running time, $\text{Time}_{inf}$. 
% The root reason behind this is that \deltagradg\ can filter out most of the unimportant training samples early by applying Theorem \ref{theorem: bound_influence} and only needs to evaluate Equation \eqref{eq: our_influence} on a few hundreds of candidate influential training samples rather than all of them. Although the set of those candidate training samples is quite small, 
In addition, we observe that \deltagradg\ always returns the same set of influential training samples as \full, which thus guarantees the correctness of \deltagradg.
% As introduced before, $\text{Time}_{inf}$ is 

\textbf{Exp3} 
%Finally, we answer \ref{q4} using the results of \textbf{Exp3} 
Experimental results of \textBF{Exp3} are shown in Figure \ref{fig:training_time}. The first observation is that \deltagradl\ can achieve up to 7.5x speed-up with respect to \retrain\ on updating the model parameters. As shown in Section \ref{sec: exp_design}, the models updated by \deltagradl\ are not exactly the same as those produced by \retrain, which might 
% Therefore, one concern is that such model differences can produce different sets of most influential samples in the sample selector, thus causing 
cause different model performance between the two methods. 
% the further deviation of the models constructed by \deltagradl\ from the ones produced by \retrain\ at the later rounds of the loop \encircle{2}. 
% be accumulated through as the \cleantwo\ proceeds, possibly hurting the model prediction performance when \deltagradl\ is used. 
However, we observe that 
% as the last two rows of Table \ref{Table: prediction_perf} indicate, 
% despite the difference of the models updated by \deltagradl\ and \retrain, 
the models constructed by those two methods have almost equivalent prediction performance (see the second to last column in Table \ref{Table: prediction_strategy}).
% after all 2000 training samples are cleaned. 
\eat{To further understand the effect of the model differences produced by those two methods, we collected the sets of influential training samples from the sample selector with \deltagradl\ and \retrain\ as implemented in the model constructor, and observe substantial overlap for all three datasets. }
This indicates that it is worthwhile to leverage \deltagradl\ for speeding up the model constructor.% phase at each iteration of the loop \encircle{2} and maintain the same prediction performance as \retrain.

==> Sections/method2.tex <==

\section{methodology}\label{sec: method}
In this section, we describe the system design in detail for the sample selector phase (Section \ref{sec: sample_selector}), the model constructor phase (Section \ref{sec: model_constructor}) and the human annotation phase (Section \ref{sec: sample_cleaner}).


\subsection{The sample selector phase}\label{sec: sample_selector}




Sample selection accomplishes two things: 1) it calculates the training sample influence using \infl\ in order to prioritize the most influential uncleaned training samples for cleaning, and simultaneously suggests possibly cleaned labels for them (see Section \ref{sec: infl}); and 2) it filters out uninfluential training samples early using \deltagradg\ at each round of loop \encircle{2} (see Section \ref{sec: deltagradg}).

\subsubsection{\infl}\label{sec: influence-l}\label{sec: infl}

The goal of \infl\ is to calculate the influence of an uncleaned training sample, $\nz$, by {estimating how much additional error will be incurred on the validation set $\mathcal{Z}_{\text{val}}$ if 1) the probabilistic label of $\nz$ is updated to some deterministic label; and 2) $\nz$ is up-weighted to 1 after it is cleaned}. % The labels in this way can be regarded as the perturbations on the labels, which,
% however, 
% However, it turns out that the original influence functions \cite{koh2017understanding} did not consider the training sample influence caused by the label changes of the labels and re-weighting the cleaned training samples. 
To capture this intuition, we propose the following modified influence function\footnote{The derivation of this formula is similar to that of the original influence function \cite{koh2017understanding}, which is included in the extended technical report \cite{wu2021chef}}:
% (see  Appendix \ref{sec: infl_derive} for the derivation):
\begin{align}\label{eq: our_influence}
\small
\begin{split}
    &\mathcal{I}_{\text{pert}}(\nz,\delta_y,\gamma) \approx N\cdot(F(\uw, \mathcal{Z}_{\text{val}}) - F(\w, \mathcal{Z}_{\text{val}}))\\
    &\hspace{-3mm} = -\nabla_\w F(\w,\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w)[\nabla_{\y}\nabla_\w F(\w,\nz)\delta_{y} + (1-\gamma) \nabla_\w F(\w,\nz)],
\end{split}
\end{align}
%how to obtain delta_y
in which $\delta_{y}$ denotes the difference between the original probabilistic label of $\nz$ and one deterministic label (ranging from 1 to $C$) and $\uw$ denotes the updated model parameters after the label is cleaned and $\nz$ is up-weighted. To calculate $\delta_{y}$, the deterministic label is first converted to its one-hot representation, i.e. a vector of length $C$ taking 1 in the $c_{th}$ entry $(c=1,2,\dots, C)$ for the label $c$ and taking 0 in all other entries (recall that $C$ represents the number of classes). 

\eat{By following the analysis of \cite{koh2017understanding}, we can derive the following formula:
\begin{align*}
\small
\begin{split}
    &\mathcal{I}_{\text{pert}}(\z,\delta_y) \approx F(\w(\delta_y), \mathcal{Z}_{\text{val}}) - F(\w, \mathcal{Z}_{\text{val}}),
\end{split}
\end{align*}
in which $\w(\delta_y)$ represents the model parameter constructed on the updated training dataset with the label of $\z$ perturbed by $\delta_y$. Therefore, Equation \eqref{eq: our_influence} can accurately quantify how the label perturbation $\delta_y$ leads to the change of the model prediction performance (represented by the loss on the validation dataset).}
% which is typically considered as a surrogate of the prediction performance.
% For two uncertain labels represented by probability vectors, $\delta_{y}$ is calculated by using the difference of those two vectors. When deterministic labels are involved in computing $\delta_{y}$, those labels are converted to their one-hot representations first, 
%how we use this influence function for solving this problem

To recommend the most influential uncleaned training samples to the human annotators and suggest possibly cleaned labels,
% how to clean their label uncertainties, 
we 1) explicitly evaluate Equation \eqref{eq: our_influence} for each uncleaned training sample for {\em all possible deterministic labels}, 2) prioritize the most ``harmful'' training samples for cleaning, i.e. the ones with the smallest negative influence values after their labels are updated to {\em some} deterministic labels, and 3) suggest those deterministic labels as the potentially cleaned labels for the human annotators. \eat{The process described above is outlined in Algorithm \ref{alg: infl}. Therefore, Equation \eqref{eq: our_influence} needs to be evaluated for $N\cdot C$ times for the entire training dataset. 

\begin{algorithm}
\small
 \caption{Compute the influence with \infl}\label{alg: infl}
 \begin{spacing}{1}
 \begin{flushleft}
 \hspace*{\algorithmicindent}
 \textbf{Input:} The input model parameter: $\w$; a training set with uncertain labels: $\mathcal{Z}_{U}$; the validation set: $\mathcal{Z}_{\text{val}}$; the cleaning budget: $b$\\
%  the Hessian-vector product: $\textbf{v}$; a set of training samples with uncertain labels: $\mathcal{Z}_{U}$; the validation dataset: $\mathcal{Z}_{\text{val}}$; the L2-norm of the class-wise hessian matrix derived at the $0_{th}$ round: $\{\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|\}_{j=1}^C$ for each $\z \in \mathcal{Z}_{U}$; the class-wise gradient: $\nabla_{\y}\nabla_\w F(\w^{(0)},\z)$ for each $\z \in \mathcal{Z}_{U}$; the cleaning budget at the current round: $b$ \\
\hspace*{\algorithmicindent} \textbf{Output:} The Top-$b$ influential training samples, $zl$, and the suggested deterministic labels for them, $yl$ \\
\end{flushleft}
 \begin{algorithmic}[1]
 \STATE Initialize a list $Infl=[]$ to contain the influence of each training sample for each deterministic label
 \STATE Initialize $zl=[], yl=[]$
\FOR{each $\z=(\x,\y) \in \mathcal{Z}_{U}$}
\FOR{$c=1$ to $C$}
% \STATE Calculate $\delta_y = y-onehot(c)$
\STATE Calculate $\mathcal{I}_{\text{pert}}(\z, \mathcal{Z}_{\text{val}},y-onehot(c))$ by using Equation \eqref{eq: our_influence} and add the result to $Infl$
\ENDFOR
\ENDFOR
\STATE Sort $Infl$ in ascending order
\STATE Go through each element, $\mathcal{I}_{\text{pert}}(\z, \mathcal{Z}_{\text{val}},\delta_y)$, in the sorted $Infl$ and add $\z,c$ to $zl,yl$ respectively if $\z$ does not appear in $zl$, which proceeds until $Len(zl)=b$
\STATE \textbf{Return} $zl$ and $yl$
% \STATE \COMMENT{\textit{The initialization step below}} 
% \STATE Pre-compute $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$ for each $\z = (\x,\y) \in \mathcal{Z}^{(0)}$ and for each class $j (j=1,2,\dots, C)$ by using Algorithm \ref{alg: pre_deltagrad}
% \STATE Pre-compute the class-wise gradient $\nabla_{\y}\nabla_\w F(\w^{(0)},\z)$ for each $\z \in \mathcal{Z}^{(0)}$
% \STATE Initialize a list, $Infl=[]$, to contain the influence of each training sample with all deterministic labels
% \STATE Initialize two lists, $zl=[]$ and $yl=[]$, to contain the Top-$b$ influential training samples and suggested deterministic labels for them
% \STATE In the {\em Sample selector}, apply \infl, i.e., Equation \eqref{eq: our_influence}, to compute the influence for each training sample $\z \in \mathcal{Z}^{(0)}$ with all possible deterministic labels $j=1,2,\dots, C$ if the label of $\z$ is uncertain, which is appended to $Infl$
% \STATE Sort $Infl$ in the {\em Sample selector} in ascending order and iterate through the sorted $Infl$ to 
% \FOR{k=1 to K}
% \STATE 
% \STATE 
% \STATE 
% \ENDFOR
  \end{algorithmic}
  \end{spacing}
  \end{algorithm}
}

\textbf{Comparison to \cite{zhang2018training}} 
As %introduced in Section \ref{sec: intro},
discussed earlier, \duti\ \cite{zhang2018training} can also recommend the most influential training samples for cleaning and suggest possibly cleaned labels, which is accomplished through solving 
a bi-level optimization problem.
% \footnote{\duti\ originally did not consider the case where the samples with deterministic and probabilistic samples have different weights. But it is straightforward to extend \duti\ to handle that.}.
% , , for detecting the most influential training samples with uncertain labels and suggesting which deterministic labels to be used to maximize the performance gains on the validation dataset. 
However, solving this problem is computationally challenging, and therefore this method cannot be used in real-time over multiple rounds (i.e. in loop \encircle{2}).
\eat{to give human annotators the most influential training samples and suggestions on how to clean their uncertain labels in real-time over multiple rounds.} 
% the human annotators thus not suitable for the scenario where repetitively detecting most influential samples is necessary. 
% Plus, as shown in , due to the difficulty of exactly solving the bi-level optimization problem when the same number of uncertain labels are cleaned, \infl\ and DUTI ends up with almost the same performance gains. 

The authors of \cite{zhang2018training} also modified the influence function to reflect the perturbations of the training labels as follows:
% (denoted as \inflg\ hereafter):
% \vspace*{-0.2cm}
\begin{align}\label{eq: prev_influence}
\small
\begin{split}
    &\mathcal{I}_{\text{pert}}(\nz) = -\nabla_\w F(\w,\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w) \nabla_{\y}\nabla_\w F(\w,\nz),
\end{split}
\end{align}
and compared it against \duti. %\ in \cite{zhang2018training}. 
% This is referred to as \inflg\ hereafter. 
Equation \eqref{eq: prev_influence}
% reflects the influence of $\z$ by adding an ``infinitely small'' perturbation on its label, which
is equivalent to removing $\delta_{y}$ (which quantifies the effect of label changes) and $(1-\gamma) \nabla_{\w} F(\w,\nz)$ from Equation \eqref{eq: our_influence}. 
% where $\delta_{y} \rightarrow 0$ follows the principle of the original influence function method \cite{koh2017understanding} by capturing the influence of the  (i.e. ). 
%However, $\delta_{y}$ can be varied in practice. 
\eat{Therefore, Equation \eqref{eq: prev_influence} may fail to quantify the model performance changes that are triggered by the label updates $\delta_y$ and is not applicable when the uncleaned training samples are down-weighted. }
As we will see in Section \ref{sec: exp}, ignoring $\delta_{y}$ in Equation \eqref{eq: prev_influence} can lead to worse performance than \infl\ even when all the training samples are equally weighted. 
% always close to 0 in practice for {\em all} training samples. 
% For example, for a binary classification task, by changing a near class-0 uncertain label, $[0.99, 0.01]$, to the class-0 label and the class-1 label respectively can lead to different magnitude of changes on labels, which are $[0.01,-0.01]$ and $[-0.99, 0.99]$ respectively. As a result, ignoring  justifies the necessity of adding the term $\delta_{y}$ in Equation \eqref{eq: our_influence}.

\textbf{Computing $\nabla_{\y}\nabla_\w F(\w,\nz)$} At first glance, it seems that the term $\nabla_{\y}\nabla_\w F(\w,\nz)$ cannot be calculated using auto-differentiation packages such as Pytorch, since it involves the partial derivative with respect to the label of $\nz$. However, we notice that this partial derivative can be explicitly calculated when the loss function $F(\w, \nz)$ is the cross-entropy function, which is the most widely used objective function in the classification task.
% \textbf{Reasonability of Equation \eqref{eq: our_influence} with large $\delta_{y}$} Note that 
% % the feasibility of 
% the partial derivative of $F(\w,\z)$ with respect to $y$ in Equation \eqref{eq: our_influence} reflects how $F(\w,\z)$ will change when {\em infinitely small} perturbations occur on $y$, which may not be suitable for the large $\delta_y$ as mentioned above. However, 
% % to reflect the differences between the predicted label and the expected label 
% for the most widely used objective function in the classification task, i.e., the cross-entropy function, $F(\w,\z)$ is a linear function of the label $y$ and thus its partial gradient with respect to $y$ is the same for all $\delta_y$. 
Specifically, the instantiation of the loss function $F(\w,\nz)$ into the cross-entropy function becomes:
% can be expressed as: 
\begin{align}\label{eq: cross_entropy_loss}
\small
\begin{split}
    F(\w, \nz) = -\sum\nolimits_{k=1}^C \ny^{(k)}\log(p^{(k)}(\w, \nx)),
\end{split}
\end{align}

In this formula above, $\ny=[\ny^{(1)}, \ny^{(2)},\dots, \ny^{(C)}]$ is the label of an input sample $\nz=(\nx,\ny)$ and $[p^{(1)}(\w, \nx), p^{(2)}(\w, \nx), \dots, p^{(C)}(\w, \nx)]$ represents the model output given this input sample, which is a probabilistic vector of length $C$ depending on the model parameter $\w$ and the input feature $\nx$.
\eat{Specifically, since given an input sample $\nz=(\nx,\ny)$, the model output is a probabilistic vector of length $C$ depending on the model parameter $\w$ and the input feature $\nx$, then the model output can be represented by $[p^{(1)}(\w, \nx), p^{(2)}(\w, \nx), \dots, p^{(C)}(\w, \nx)]$. By further representing $\ny$ as $\ny=[\ny^{(1)}, \ny^{(2)},\dots, \ny^{(C)}]$, the instantiation of the loss function $F(\w,\nz)$ into the cross-entropy function can be expressed as: 
\begin{align*}
\small
\begin{split}
    F(\w, \nz) = -\sum\nolimits_{k=1}^C \ny^{(k)}\log(p^{(k)}(\w, \nx)),
\end{split}
\end{align*}}
Then we can observe that Equation \eqref{eq: cross_entropy_loss} is a linear function of the label $\ny$. 
% Therefore, the partial derivative of $F(\w, \z)$ with respect to $y$ is free of $y$ and suitable for an arbitrary perturbation, $\delta_y$.
% and a large perturbation $\delta_y$ in Equation \eqref{eq: our_influence} is an accurate quantification of the influence upon changing the $y$ by an arbitrary $\delta_y$. 
Hence, $\nabla_{\y}\nabla_\w F(\w,\nz)$ can be explicitly evaluated as:
\begin{align}\label{eq: class_wise_grad}
\small
    \begin{split}
\nabla_{\y}\nabla_\w F(\w,\nz) = [-\nabla_{\w} \log(p^{(1)}(\w, \nx)), \dots, -\nabla_{\w} \log(p^{(C)}(\w, \nx))]        
    \end{split}
\end{align}
As a result, each $-\nabla_{\w} \log(p^{(c)}(\w, \nx)),c=1,2,\dots, C$ can be calculated with the auto-differentiation package.

\textbf{Computing $\bH^{-1}(\w)$} Recall that $\bH(\w)$ denotes the Hessian matrix averaged on all training samples. Rather than explicitly calculating its inverse, 
% which is very time-consuming, 
by following \cite{koh2017understanding}, we leverage the conjugate gradient method \cite{martens2010deep} to approximately compute the Matrix-vector product $\nabla_\w F(\w,\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w)$ in Equation \eqref{eq: our_influence}. 

\subsubsection{\deltagradg}\label{sec: deltagradg} The goal of using \infl\ is to quantify the influence of all uncleaned training samples and select the Top-$b$ influential training samples for cleaning. But in loop \encircle{2}, this search space could be reduced by employing \deltagradg. 
% To avoid repetitively evaluating Equation \eqref{eq: our_influence} 
Specifically, other than the initialization step, we can leverage {\em \deltagradg} to prune away most of the uninfluential training samples early in following rounds, thus only evaluating the influence of a small set of candidate influential training samples in those rounds.
\eat{Specifically, we can evaluate the influence of every training sample in the initialization step with Equation \eqref{eq: our_influence} and then leverage {\em \deltagradg} to filter out the uninfluential training samples early, thus only evaluating the influence of a small set of candidate influential training samples in following rounds. }
Suppose this set of samples is denoted as $\mathcal{Z}_{inf}^{(k)}$ for the round $k$; the derivation of this set is outlined in Algorithm \ref{alg: deltagradg}. 
As this algorithm indicates, the first step is 
% As the first step toward obtaining $\mathcal{Z}_{inf}^{(k)}$, 
% The intuition of \deltagradg\ is that prior to evaluating the expensive Equation \eqref{eq: our_influence} on any training sample, 
% we need 
to effectively estimate the maximal perturbations of Equation \eqref{eq: our_influence} at the $k_{th}$ cleaning round for each uncleaned training sample $\nz$ and each possible label change $\delta_y$ (see line \ref{line: cal_perturbation}),
% (see lines \ref{line: bound_start} to \ref{line: bound_end}),
%in Algorithm \ref{alg: deltagradg}),
which are assumed to take $\mathcal{I}_0(\nz, \delta_y, \gamma)$ (see Theorem \ref{theorem: bound_influence} for its definition) as the perturbation center.
% and take $ub^{(k)}(\z, \delta_y)$ and $lb^{(k)}(\z, \delta_y)$ as the upper and lower bound, respectively. 
Then the first part of $\mathcal{Z}_{inf}^{(k)}$ consists of all the training samples which produce the Top-$b$ smallest values of $\mathcal{I}_0(\nz, \delta_y, \gamma)$ with a given $\delta_y$ (see line 6).
%of Algorithm~\ref{alg: deltagradg} for how this is calculated). 
For those $b$ smallest values, we also collect the maximal value of their upper bound, $L$. We then include in $\mathcal{Z}^{(k)}_{inf}$ all the remaining training samples whose lower bound, is smaller than $L$ with certain $\delta_y$ (see line \ref{line: second_z_k}).
%in Algorithm \ref{alg: deltagradg}).
This indicates the possibility of those samples becoming the Top-$b$ influential samples. 
% The process to obtain $\mathcal{Z}^{(k)}_{inf}$ is also intuitively explained in Appendix \ref{sec: increm_infl_explanations}. 
% We analyze the time complexity of using \deltagradg\ to select the most influential training samples in . 

As described above, it is critical to estimate the maximal perturbation of Equation \eqref{eq: our_influence} for each uncleaned training sample, $\nz$, and each label perturbation, $\delta_y$,
%as the first step to obtain $\mathcal{Z}^{(k)}_{inf}$, 
which requires the following theorem. 
% We The intuitive idea of removing those influential  
% which are assumed to be $lb^{(k)}$ between the $k_{th} (k>1)$ round and the initialization step, which is assumed to be perturbed around  . 

% With these changes in hand, we can then identify the uninfluential training samples by quantifying 

% , which relies on the following theorem.
\eat{
\begin{theorem}\label{theorem: bound_influence}
For a training sample $\nz={(\nx, \ny)}$ which has not been cleaned before the $k$ rounds of loop \encircle{2}, the following bounds hold for Equation \eqref{eq: our_influence} evaluated on the training sample $\nz$ and a label perturbation $\delta_y$ at the $k_{th}$ round:
% (denoted as $\mathcal{I}^{(k)}_{\text{pert}}(\z, \delta_y)$):
\begin{align*}
\small
\begin{split}
    & |\mathcal{I}^{(k)}_{\text{pert}}(\nz,\delta_y,\gamma) - \mathcal{I}_0(\nz, \delta_y, \gamma) - \frac{1-\gamma}{2}e_1\mu - \sum_{j=1}^C \delta_{y,j}e_1 \|\bH^{(j)}(\w^{(k)}, \nz)\||\\
    & \leq \sum_{j=1}^C |\delta_{y,j}|e_2
    % \mathbf{I}[\delta_{y,j} < 0](e_1 - e_2) + \mathbf{I}[\delta_{y,j} \geq 0](e_1 + e_2)]
    \|\bH^{(j)}(\w^{(k)}, \nz)\| + \frac{1-\gamma}{2}e_2\mu\\
    % &\mathcal{I}^{(k)}_{\text{pert}}(\nz, \delta_y) 
    % = -\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)}) \nabla_{\y}\nabla_\w F(\w^{(k)},\z)\delta_{y} \\
    % & \in [lb^{(k)}(\z, \delta_y), ub^{(k)}(\z, \delta_y)]\\
    % % & = [ - \pbound^{(k)}(\z,\delta_y), \pcenter^{(k)}(\z, \delta_y) + \pbound^{(k)}(\z,\delta_y)]
    % & = [\sum_{j=1}^C \delta_{y,j}[\mathbf{I}[\delta_{y,j} < 0]e_1 + \delta_{y,j} \geq 0]e_2]\|\bH^{(j)}(\w^{(k)}, \z)\|, \\
    % & \sum_{j=1}^C \delta_{y,j}[\mathbf{I}[\delta_{y,j} < 0]e_2 + \delta_{y,j} \geq 0]e_1]\|\bH^{(j)}(\w^{(k)}, \z)\|] %+ \frac{1-\gamma}{2}e_2\|\int_{0}^1 \bH(\w^{(0)} + s(\w^{(k)} - \w^{(0)}), \z) ds\|, ]
    % \pcenter^{(k)}(\z, \delta_y) + \pbound^{(k)}(\z, \delta_y)\\ 
    % \textbf{v}\nabla_{\y}\nabla_\w F(\w^{(0)},\z)\delta_{y} +\frac{1}{2}\sum\nolimits_{j=1}^C \delta_{y,j} \textbf{v}^\top(\w^{(k)} - \w^{(0)}) \|\bH^{(j)}(\w^{(0)}, \w^{(k)}, \z)\|\\
    % & +  \frac{1}{2}\sum\nolimits_{j=1}^C |\delta_{y,j}|\|\textbf{v}\|\|(\w^{(k)} - \w^{(0)})\| \|\bH^{(j)}(\w^{(0)}, \w^{(k)}, \z)\|,\\
% \end{split}
% \end{align*}
% \begin{align*}
% \small
% \begin{split}
    %     &\mathcal{I}^{(k)}_{\text{pert}}(\z, \delta_y) = -\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)}) \nabla_{\y}\nabla_\w F(\w^{(k)},\z)\delta_{y} \\
    % & \geq \pcenter^{(k)}(\z, \delta_y) - \pbound^{(k)}(\z, \delta_y)
    % & - \frac{1}{2}\sum\nolimits_{j=1}^C |\delta_{y,j}|\|\textbf{v}\|\|(\w^{(k)} - \w^{(0)})\| \|\bH^{(j)}(\w^{(0)}, \w^{(k)}, \z)\|
\end{split}
\end{align*}
in which, $\textbf{v}^\top = -\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)})$,
% \frac{1}{2}\sum\nolimits_{j=1}^C \delta_{y,j} \textbf{v}^\top(\w^{(k)} - \w^{(0)}) \|\bH^{(j)}( \w^{(k)}, \z)\|+ \textbf{v}\nabla_{\y}\nabla_\w F(\w^{(0)},\z)\delta_{y}$,
% $\pbound^{(k)}(\z, \delta_y) = \frac{1}{2}\sum\nolimits_{j=1}^C |\delta_{y,j}|\|\textbf{v}\|\|\bH^{(j)}(\w^{(k)}, \z)\|\|\w^{(k)} - \w^{(0)}\|$, 
% $\textbf{v}^\top = -\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)}),$
$\delta_{y} = [\delta_{y,1}, \delta_{y,2},\dots, \delta_{y,C}]$,
$\bH^{(j)}(\w^{(k)}, \nz) = \int_{0}^1 -\nabla_{\w}^2\log(p^{(j)}(\w^{(0)} + s(\w^{(k)} - \w^{(0)}), \nx)) ds$, $\mu = \|\int_{0}^1 \bH(\w^{(0)} + s(\w^{(k)} - \w^{(0)}), \nz) ds\|$,
$e_1 = \textbf{v}^\top(\w^{(k)} - \w^{(0)})$, $e_2 = \|\textbf{v}\|\|\w^{(k)} - \w^{(0)}\|$ and $\mathcal{I}_0(\nz, \delta_y, \gamma) = \textbf{v}^\top[\nabla_{\y}\nabla_\w F(\w^{(0)},\nz)\delta_{y} + (1-\gamma) \nabla_\w F(\w^{(0)},\nz)]$.
% \begin{align*}
% \small
% \begin{split}
% &\pcenter^{(k)}(\z, \delta_y) = \frac{1}{2}\sum\nolimits_{j=1}^C \delta_{y,j} \textbf{v}^\top(\w^{(k)} - \w^{(0)}) \|\bH^{(j)}( \w^{(k)}, \z)\|\\    
% & + \textbf{v}\nabla_{\y}\nabla_\w F(\w^{(0)},\z)\delta_{y},\\
% & \pbound^{(k)}(\z, \delta_y) = \frac{1}{2}\sum\nolimits_{j=1}^C |\delta_{y,j}|\|\textbf{v}\|\|\w^{(k)} - \w^{(0)}\| \|\bH^{(j)}(\w^{(k)}, \z)\|,\\
% & \textbf{v}^\top = -\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)}),\delta_{y} = [\delta_{y,1}, \delta_{y,2},\dots, \delta_{y,C}],\\
% & \bH^{(j)}(\w^{(k)}, \z) = \int_{0}^1 -\nabla_{\w}^2\log(p^{(j)}(\w^{(0)} + s(\w^{(k)} - \w^{(0)}), \x)) ds
% \end{split}
% \end{align*}
% $\mathcal{I}_0(\z, \mathcal{Z}_{\text{val}}, \delta_y) = \textbf{v}\nabla_{\y}\nabla_\w F(\w^{(0)},\z)\delta_{y}$, 
\end{theorem}
}
%\scream{Reformatted Theorem, it was not readable.}
\begin{theorem}\label{theorem: bound_influence}
For a training sample $\nz={(\nx, \ny)}$ which has not been cleaned before the $k^{th}$ round of loop \encircle{2}, the following bounds hold for Equation \eqref{eq: our_influence} evaluated on the training sample $\nz$ and a label perturbation $\delta_y$:
\begin{align*}
\small
\begin{split}
    & |-\mathcal{I}^{(k)}_{\text{pert}}(\nz,\delta_y,\gamma) - \mathcal{I}_0(\nz, \delta_y, \gamma) - \frac{1-\gamma}{2}e_1\mu - \sum\nolimits_{j=1}^C \delta_{y,j}e_1 \|\bH^{(j)}(\w^{(k)}, \nz)\||\\
    & \leq \sum\nolimits_{j=1}^C |\delta_{y,j}|e_2
    \|\bH^{(j)}(\w^{(k)}, \nz)\| + \frac{1-\gamma}{2}e_2\mu,
\end{split}
\end{align*}

in which, $\mathcal{I}_0(\nz, \delta_y, \gamma) = \textbf{v}^\top[\nabla_{\y}\nabla_\w F(\w^{(0)},\nz)\delta_{y} + (1-\gamma) \nabla_\w F(\w^{(0)},\nz)]$,
$\textbf{v}^\top = -\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)})$,
$\delta_{y} = [\delta_{y,1}, \delta_{y,2},\dots, \delta_{y,C}]$,\\
$\bH^{(j)}(\w^{(k)}, \nz) = \int_{0}^1 -\nabla_{\w}^2\log(p^{(j)}(\w^{(0)} + s(\w^{(k)} - \w^{(0)}), \nx)) ds$, \\
$\mu = \|\int_{0}^1 \bH(\w^{(0)} + s(\w^{(k)} - \w^{(0)}), \nz) ds\|$, and\\
$e_1 = \textbf{v}^\top(\w^{(k)} - \w^{(0)})$, $e_2 = \|\textbf{v}\|\|\w^{(k)} - \w^{(0)}\|$.
\end{theorem}


To reduce the computational overhead, 
% the perturbation of the influence value $\mathcal{I}^{(k)}_{\text{pert}}(\z, \delta_y)$ is centered around the value $\pcenter^{(k)}(\z, \delta_y)$ and has an upper bound of $\pbound^{(k)}(\z, \delta_y)$. 
% for deriving the bound of $\mathcal{I}^{(k)}_{\text{pert}}(\z, \mathcal{Z}_{\text{val}},\delta_y)$ in the above theorem, 
the integrated Hessian matrices, $\int_{0}^1 \bH(\w^{(0)} + s(\w^{(k)} - \w^{(0)}), \nz) ds$ and $\bH^{(j)}(\w^{(k)}, \nz)$, are approximated by their counterparts evaluated at $\w^{(0)}$, i.e., $\bH(\w^{(0)}, \nz)$ and $-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx))$.
% , which can be pre-computed in the initialization step. 
% Due to this approximation, we can observe that 
As a consequence, the bounds 
% on $\mathcal{I}^{(k)}_{\text{pert}}(\z, \mathcal{Z}_{\text{val}},\delta_y)$ in Theorem \ref{theorem: bound_influence} 
can be calculated by applying several linear algebraic operations on $\textbf{v}$, $\w^{(k)}$, $\w^{(0)}$ 
% according to Theorem \ref{theorem: bound_influence}, to derive the upper bound and lower bound of $\mathcal{I}^{(k)}_{\text{pert}}(\z, \mathcal{Z}_{\text{val}})$, we can pre-compute 
and some pre-computed formulas, i.e., the norm of the Hessian matrices,  $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx))\|$ and $\|\bH(\w^{(0)}, \nz)\|$, and the gradients, $\nabla_{\y}\nabla_\w F(\w^{(0)},\nz)$ and $\nabla_\w F(\w^{(0)},\nz)$, which can be computed as ``provenance'' information in the initialization step. Note that pre-computing $\nabla_{\y}\nabla_\w F(\w^{(0)},\nz)$ and $\nabla_\w F(\w^{(0)},\nz)$ is quite straightforward by leveraging Equation \eqref{eq: class_wise_grad}. Then the remaining question is how to compute $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx))\|$ and $\|\bH(\w^{(0)}, \nz)\|$ efficiently without explicitly evaluating the Hessian matrices. Since those two terms calculate the norm of one Hessian matrix, we therefore only take one of them as a running example to describe how to compute them in a feasible way, as shown below.

% \textbf{Pre-computing $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx))\|$} 
\textbf{Pre-computing $\|\bH(\w^{(0)}, \nz)\|$} 
% In Algorithm \ref{alg: deltagradg}, its input includes the pre-computed formulas ini the initialization step, i.e., the L2-norm of the class-wise hessian matrix, $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$ and the class-wise gradient, $\nabla_{\y}\nabla_\w F(\w^{(0)},\z)$. Computing the latter term is easy since we can simply cache it for each training sample and each class during the initialization step. To obtain the value of $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$, 
Since 1) a Hessian matrix is symmetric (due to its positive definiteness); and 2) the L2-norm of a symmetric matrix is equivalent to its eigenvalue with the largest magnitude \cite{meyer2000matrix}, the L2 norm of one Hessian matrix is thus equivalent to its largest eigenvalue. 
% can be derived by calculating its largest eigenvalue in magnitude
% Obviously it would be very expensive to calculate this term through explicitly evaluating the Hessian matrix. 
To evaluate this eigenvalue, 
% the L2 norm of
% $-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx))$
% $\bH(\w^{(0)}, \nz)$
we use the Power method \cite{golub2000eigenvalue}, which is discussed in the extended technical report \cite{wu2021chef}.
% Appendix \ref{sec: hessian norm}. 
% Due to space limit, the algorithmic details of invoking the Power method this step is included in 
\eat{In addition, we note that the power method involves computing the product between the Hessian matrix 
% $-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx))$ 
$\bH(\w^{(0)}, \nz)$ and a vector $\textbf{g}$,
% As mentioned in \cite{do2007efficient}, the Hessian-vector product 
which can be effectively calculated with the auto-differentiation package, such as Pytorch (see Appendix \ref{sec: hessian-vec product} for details).  }
\eat{the following equation, without explicitly computing the full Hessian matrix:
% \begin{align}\label{eq: hessian_vector_prod}
% \small
% \begin{split}
%     & -\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx)) \textbf{g}\\
%     % & \bH^{(j)}(\w^{(0)}, \z)\textbf{g}\\
%     &= \lim_{s\rightarrow 0}\frac{-\nabla_{\w}\log(p^{(j)}(\w^{(0)} + s \textbf{g}, \nx)) - [-\nabla_{\w}\log(p^{(j)}(\w^{(0)}, \nx))]}{s},
%     % & = \lim_{s\rightarrow 0}\frac{\bH^{(j)}(\w^{(0)} + s \textbf{g}, \z), \x)) - \bH^{(j)}(\w^{(0)}, \z)}{s},
% \end{split}
% \end{align}
\begin{align}\label{eq: hessian_vector_prod}
\small
\begin{split}
    & \bH(\w^{(0)}, \nz)\textbf{g}= \lim_{s\rightarrow 0}\frac{\bH(\w^{(0)} + s \textbf{g}, \nz) - \bH(\w^{(0)}, \nz)}{s},
    % & = \lim_{s\rightarrow 0}\frac{\bH^{(j)}(\w^{(0)} + s \textbf{g}, \z), \x)) - \bH^{(j)}(\w^{(0)}, \z)}{s},
\end{split}
\end{align}
in which $s$ is a scalar. In the implementation, we approximately evaluate Equation \eqref{eq: hessian_vector_prod} by setting $s$ as a near-zero constant (e.g. $1e^{-6}$). }

\textbf{Time complexity of \deltagradg} By assuming that there are $n$ samples left after \deltagradg\ is used, the dimension of vectorized $\w$ is $m$, and the running time of computing the vector $\textbf{v}$ and the gradient ($\nabla_{\y}\nabla_\w F(\w,\nz)$ or $\nabla_\w F(\w,\nz)$) is denoted by $O(v)$ and $O(\text{Grad})$ respectively, the time complexity of \deltagradg\ is $O(v) + NC(O(Cm) + O(m) + O(C)) + nc O(\text{Grad})$ (see the extended technical report \cite{wu2021chef} for detailed analysis).
% We summarize the subroutine for pre-computing $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$ in Algorithm \ref{alg: pre_deltagrad}.

\eat{
\begin{algorithm}
\small
 \caption{Pre-compute $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$ in the initialization step}\label{alg: pre_deltagrad}
 \begin{spacing}{1}
 \begin{flushleft}
 \hspace*{\algorithmicindent}
 \textbf{Input:} A training sample $\z \in \mathcal{Z}$, the class $j$ and the model parameter obtained in the initialization step: $\w^{(0)}$\\
\hspace*{\algorithmicindent} \textbf{Output:} $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$. 
\end{flushleft}
 \begin{algorithmic}[1]
 
 
 
% \STATE Initialize $\mathcal{Z}^{(k)}_{inf} = \{\}$
% \STATE Initialize two lists $LB=[], UB=[]$, representing the lower bound and upper bound of the influence of each sample.
% \STATE Initialize one list $Infl=[]$ to include the value of $\textbf{v}\nabla_{\y}\nabla_\w F(\w^{(0)},\z)\delta_{y}$ for all the sample $\z in \mathcal{Z}_U$
% \STATE Calculate $\textbf{v}=-\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)})$ by using the Hessian-vector product algorithm from \cite{koh2017understanding}.
  % I want the below text to be left 
  % "Some text before the logic:"
%   \FOR{each $\z \in \mathcal{Z}$}
   \STATE Initialize $\textbf{g}$ as a random vector;
   \STATE \COMMENT{\textit{Power method below}}
   \WHILE{\textbf{g} is not converged} 
    \STATE Calculate $-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\textbf{g}$ by using Equation \eqref{eq: hessian_vector_prod}
    \STATE Update $\textbf{g}$: $\textbf{g}=\frac{-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\textbf{g}}{\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\textbf{g}\|}$
   \ENDWHILE 
   \STATE Calculate the largest eigenvalue of $-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))$ in magnitude by using $ \frac{\textbf{g}\cdot (-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\textbf{g})}{\|\textbf{g}\|}$, which is equivalent to $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$.
%   \FOR{each deterministic label $c \in \{1,2,\dots, C\}$}
%     \STATE Denote $\delta_y = y - onehot(c)$
%     \STATE Calculate $\textbf{v}\nabla_{\y}\nabla_\w F(\w^{(0)},\z)\delta_{y}$ and add the result to the list $Infl$
%      \STATE Calculate the upper bound and lower bound of $\mathcal{I}^{(k)}_{\text{pert}}(\z, \mathcal{Z}_{\text{val}},\delta_y)$ (denoted as $lb(\z,\delta_y)$ and $ub(\z,\delta_y)$) by using Theorem \ref{theorem: bound_influence}.
%      Add $lb(\z,\delta_y)$ to $LB$ and add $ub(\z,\delta_y)$ to $UB$
%      \ENDFOR
%   \ENDFOR 
    % \STATE sort $Infl$ in ascending order and denote the sorted list as $sInfl$
    % \STATE For the first $b$ entries in $sInfl$, add the corresponding training samples to $\mathcal{Z}^{(k)}_{inf}$
    % \STATE For the remaining entries in $sInfl$, add the training samples to $\mathcal{Z}^{(k)}_{inf}$, which have one entry in $sInfl$ whose lower bound is larger than the upper bound of at least one entry within the first $b$ entries.
    \STATE \textbf{Return} $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$.
  % I want the below text to be left 
%   \algotext{Some text before the logic:}

  % Here I want the numbering to start from 1 again
  \end{algorithmic}
  \end{spacing}
  \end{algorithm}
}
% \textbf{Filtering out uninfluential training samples} With the bound on $\mathcal{I}^{(k)}_{\text{pert}}(\z, \delta_y)$ in hand for all uncleaned training samples, we can then determine all the {\em candidate training samples}, $\mathcal{Z}^{(k)}_{inf}$, which are likely to become Top-$b$ influential at the $k_{th}$ round of the loop \encircle{2}, and thus filter out all the other training samples. The first part of $\mathcal{Z}^{(k)}_{inf}$ consists of all the training samples which produce the Top-$b$ smallest values of $\pcenter^{(k)}(\z, \delta_y)$ with a given $\delta_y$ (see line 6 of Algorithm~\ref{alg: deltagradg} for how this is calculated). 
% Then we obtain the largest value of $\pcenter^{(k)}(\z, \delta_y) + \pbound^{(k)}(\z, \delta_y)$ (denoted by $L$) among those training samples, which represents the maximal possible value of $\mathcal{I}^{(k)}_{\text{pert}}(\z, \delta_y)$ that those samples can reach. Then we include all the other training samples whose lower bound, $\pcenter^{(k)}(\z, \delta_y) - \pbound^{(k)}(\z, \delta_y)$, is smaller than $L$ with certain $\delta_y$ into $\mathcal{Z}^{(k)}_{inf}$. This indicates the possibility of those samples becoming the Top-$b$ influential samples. 
% % by utilizing the largest lower bound,  among all the first part of the candidate training samples, $L$, the second part consists of the other training samples which can have the upper bound of the influence value smaller than $L$.
% This process is then summarized in Algorithm \ref{alg: deltagradg} and intuitively illustrated in Figure \ref{fig:deltagradg}. 




% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output\,}
% \SetKwInOut{Data}{Data}
% \SetKwProg{Tree}{Tree}{}{EndTree}

% \begin{algorithm}[H]
%   \caption{The ASP\_Tree algorithm}
%   \Input{TV database and min\_sup}
%   \Output{Bla bla bla}
%   \Data{bla bla bla}
%   \Tree{$TV_i, min\_sup$}{
%     $[\text{Root}] \gets [\text{NULL}]$\;
%     \For {$i = 1$ to $N$} {
%       $\text{Root} \gets TV_1$\;
%       $i \gets i + 1$\;
%       \uIf {$TV_i > \textup{Root}$}{
%         $\text{Root} \gets TV_i$\;}
%       \uElseIf{$TV_i \leq \textup{Root}$}{
%         $i \gets i+1$\;}
%       \Else{
%         do something interesting\;
%       }
%     }
%   }
% \end{algorithm}

\eat{
\begin{algorithm}
\small
 \caption{\deltagradg}\label{alg: deltagradg}
 \begin{spacing}{1}
 \begin{flushleft}
 \hspace*{\algorithmicindent}
 \textbf{Input:} 
%  The model parameter constructed at the $k_{th}$ round: $\w^{(k)}$; the Hessian-vector product: $\textbf{v}$; 
 a set of uncleaned training samples: $\mathcal{Z}_{U}$; the validation dataset: $\mathcal{Z}_{\text{val}}$; 
%  the L2-norm of the Hessian matrix and the class-wise Hessian matrix derived
 Pre-computed information at the initialization step: $\|\bH(\w^{(0)}, \nz)\|$, $\{\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx))\|\}_{j=1}^C$ for each $\nz \in \mathcal{Z}_{U}$ and the class-wise gradient: $\nabla_{\y}\nabla_\w F(\w^{(0)},\nz)$ for each $\nz \in \mathcal{Z}_{U}$; \# of samples to be cleaned at the current round: $b$ \\
\hspace*{\algorithmicindent} \textbf{Output:} A set of prioritized training samples for cleaning: $\mathcal{Z}^{(k)}_{inf}$ 
\end{flushleft}
 \begin{algorithmic}[1]
\STATE Initialize $\mathcal{Z}^{(k)}_{inf} = \{\}$
% \STATE Initialize two lists $LB=[], UB=[]$, representing the lower bound and upper bound of the influence of each uncleaned sample.
\STATE Initialize one list $Infl=[]$% to include the value of $\pcenter$ for all $\nz \in \mathcal{Z}_U$
% \STATE Calculate $\textbf{v}=-\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)})$ by using the Hessian-vector product algorithm from \cite{koh2017understanding}.
  % I want the below text to be left 
  % "Some text before the logic:"
   \FOR{each $\nz=(\nx,\ny) \in \mathcal{Z}_{U}$ and each deterministic label $c \in \{1,2,\dots, C\}$}
%   \FOR{each deterministic label $c \in \{1,2,\dots, C\}$}
    \STATE Denote $\delta_y = y - onehot(c)$ \label{line: bound_start}
    \STATE Calculate $\mathcal{I}_0(\nz, \delta_y, \gamma)$ and add the result to the list $Infl$
     \STATE Calculate the bound on $\mathcal{I}^{(k)}_{\text{pert}}(\nz,\delta_y,\gamma)$     %  of $\mathcal{I}^{(k)}_{\text{pert}}(\z, \delta_y)$ % (denoted as $lb(\z,\delta_y)$ and $ub(\z,\delta_y)$) 
     by using Theorem \ref{theorem: bound_influence}\label{line: bound_end}.
    %  and add them to $UB$ and $LB$ respectively 
    %  \ENDFOR
   \ENDFOR 
   \STATE identify the Top-$b$ smallest items in $infl$, add 
    % \STATE sort $Infl$ in ascending order, (denoted by $[\pcenter_1, \pcenter_2,\pcenter_3, \dots]$, add 
    the corresponding training samples 
    % of the first $b$ entries in this sorted list 
    to $\mathcal{Z}^{(k)}_{inf}$ and obtain the largest upper bound, $L$, among those items \label{line: first_z_k}
    % \STATE 
    \STATE For the remaining training samples, if the lower bound of their influence is smaller than $L$ with a certain $\delta_y$, add them to $\mathcal{Z}^{(k)}_{inf}$ \label{line: second_z_k}
    % , which have one entry in $sInfl$ whose lower bound is larger than the upper bound of at least one entry within the first $b$ entries.
    \STATE \textbf{Return} $\mathcal{Z}^{(k)}_{inf}$%and $\textbf{v}$.
  % I want the below text to be left 
%   \algotext{Some text before the logic:}

  % Here I want the numbering to start from 1 again
  \end{algorithmic}
  \end{spacing}
  \end{algorithm}
}
\begin{algorithm}
\small
 \caption{\deltagradg}\label{alg: deltagradg}
 \begin{spacing}{1}
 \begin{flushleft}
 \hspace*{\algorithmicindent}
 \textbf{Input:} 
%  The model parameter constructed at the $k_{th}$ round: $\w^{(k)}$; the Hessian-vector product: $\textbf{v}$; 
%  a set of uncleaned training samples: $\mathcal{Z}_{U}$; the validation dataset: $\mathcal{Z}_{\text{val}}$; 
% %  the L2-norm of the Hessian matrix and the class-wise Hessian matrix derived
%  Pre-computed information at the initialization step: $\|\bH(\w^{(0)}, \nz)\|$, $\{\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \nx))\|\}_{j=1}^C$ for each $\nz \in \mathcal{Z}_{U}$ and the class-wise gradient: $\nabla_{\y}\nabla_\w F(\w^{(0)},\nz)$ for each $\nz \in \mathcal{Z}_{U}$; 
 The number of samples to be cleaned at the $k_{th}$ round: $b$ \\
\hspace*{\algorithmicindent} \textbf{Output:} A set of prioritized training samples for cleaning: $\mathcal{Z}^{(k)}_{inf}$ 
\end{flushleft}
 \begin{algorithmic}[1]
\STATE Initialize $\mathcal{Z}^{(k)}_{inf} = \{\}$
% \STATE Initialize two lists $LB=[], UB=[]$, representing the lower bound and upper bound of the influence of each uncleaned sample.
% \STATE Initialize one list $Infl=[]$% to include the value of $\pcenter$ for all $\nz \in \mathcal{Z}_U$
% \STATE Calculate $\textbf{v}=-\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)})$ by using the Hessian-vector product algorithm from \cite{koh2017understanding}.
  % I want the below text to be left 
  % "Some text before the logic:"
  \STATE Calculate $\mathcal{I}_0(\nz, \delta_y, \gamma)$ and the perturbation bound on this term by using Theorem \ref{theorem: bound_influence} for each uncleaned sample, $\nz=(\nx,\ny)$, and each label perturbation, $\delta_y=\ny - onehot(c), (c=1,2,\dots, C)$ \label{line: cal_perturbation}
%   \FOR{each $\nz=(\nx,\ny) \in \mathcal{Z}_{U}$ and each deterministic label $c \in \{1,2,\dots, C\}$}
% %   \FOR{each deterministic label $c \in \{1,2,\dots, C\}$}
%     \STATE Denote $\delta_y = y - onehot(c)$ \label{line: bound_start}
%     \STATE Calculate $\mathcal{I}_0(\nz, \delta_y, \gamma)$ and add the result to the list $Infl$
%      \STATE Calculate the bound on $\mathcal{I}^{(k)}_{\text{pert}}(\nz,\delta_y,\gamma)$     %  of $\mathcal{I}^{(k)}_{\text{pert}}(\z, \delta_y)$ % (denoted as $lb(\z,\delta_y)$ and $ub(\z,\delta_y)$) 
%      by using Theorem \ref{theorem: bound_influence}\label{line: bound_end}.
%     %  and add them to $UB$ and $LB$ respectively 
%     %  \ENDFOR
%   \ENDFOR 
   \STATE 
%   identify the Top-$b$ smallest items in $infl$,
   Add the training samples producing Top-$b$ smallest $\mathcal{I}_0(\nz, \delta_y, \gamma)$ to $\mathcal{Z}^{(k)}_{inf}$
    % \STATE sort $Infl$ in ascending order, (denoted by $[\pcenter_1, \pcenter_2,\pcenter_3, \dots]$, add 
    % of the first $b$ entries in this sorted list
   \STATE obtain the largest perturbation upper bound, $L$, for all Top-$b$ smallest $\mathcal{I}_0(\nz, \delta_y, \gamma)$\label{line: first_z_k}
    % \STATE 
    \STATE For any remaining training sample, $\nz$, if its lower perturbation bound of $\mathcal{I}_0(\nz, \delta_y, \gamma)$ is smaller than $L$ with a certain $\delta_y$, add it to $\mathcal{Z}^{(k)}_{inf}$ \label{line: second_z_k}
    % , which have one entry in $sInfl$ whose lower bound is larger than the upper bound of at least one entry within the first $b$ entries.
    \STATE \textbf{Return} $\mathcal{Z}^{(k)}_{inf}$%and $\textbf{v}$.
  % I want the below text to be left 
%   \algotext{Some text before the logic:}

  % Here I want the numbering to start from 1 again
  \end{algorithmic}
  \end{spacing}
  \end{algorithm}




\subsection{The model constructor phase (\deltagradl)}\label{sec: model_constructor}

% \begin{algorithm}%[h!] 
% \small
% % \footnotesize
% \begin{flushleft}
% % \SetKwInOut{Input}{Input}
% % \SetKwInOut{Output}{Output}
% \textbf{Input: }{The full training set $\mathcal{Z}$, model parameters cached in the last iteration $k$, $\{\w_{0}^{(k)}, \w_{1}^{(k)}, \dots, \w_{t}^{(k)}\}$ and corresponding gradients $\{\nabla F\left(\w_{0}^{(k)},\miniB_0\right), \nabla F\left(\w_{1}^{(k)},\miniB_1\right), \dots, \nabla F\left(\w_{t}^{(k)},\miniB_t\right)\}$, the indices of the cleaned training samples $\mathcal{R}^{(k)}$ at the $k_{th}$ iteration and their updated labels, learning rate $\eta_t$, total training iteration number $T$, the hyper-parameters used in \deltagrad: $m$, $j_0$ and $T_0$}


% \textbf{Output: }{Updated model parameter $\w_{T}^{(k+1)}$}
% \end{flushleft}
%  \begin{algorithmic}[1]
% \STATE Initialize $\w_{0}^{(k+1)} \leftarrow \w_{0}^{(k)}$

% \STATE Initialize an array $\Delta G = \left[\right]$

% \STATE Initialize an array $\Delta W = \left[\right]$

% \FOR{$t=0;t<T; t++$}{

% \IF{$[((t-j_0) \mod T_0) == 0]$ or $t \leq j_0$}
% {
%     \STATE compute $\nabla F\left(\w_{t}^{(k+1)};\miniB_t \right)$ exactly with the updated labels on $\miniB_t \bigcap R$
    
%     \STATE compute $\nabla F\left(\w_{t}^{(k+1)};\miniB_t\right) - \nabla F\left(\w_{t}^{(k)};\miniB_t \right)$
    
%     \STATE set $\Delta G\left[r\right] = \nabla F\left(\w_{t}^{(k+1)};\miniB_t\right) - \nabla F\left(\w_{t}^{(k)};\miniB_t\right)$
    
%     \STATE set $\Delta W\left[r\right] = \w_{t}^{(k+1)} - \w_{t}^{(k)}$%, based on the cached parameters $\w_{t}$
%     , $r\leftarrow r+1$
    
%     \STATE compute $\w_{t+1}^{(k+1)}$: $\w_{t+1}^{(k+1)} \leftarrow \w_{t}^{(k+1)} - \eta_t \nabla F\left(\w_{t}^{(k+1)};\miniB_t \right)$
% }
% \ELSE
% {
%     \STATE Pass $\Delta W\left[-m:\right]$, $\Delta G\left[-m:\right]$, i.e., the last $m$ elements in $\Delta W$ and $\Delta G$, and 
%     % which are from the $j_1^{th}, j_2^{th},\dots, j_m^{th}$ iterations where $j_1 < j_2< \dots < j_m$ depend on $t$, 
%     $\textbf{v} = \iw_{t} - \w_{t}$
%     % and the history size $m$, 
%     to the L-BFGFS Algorithm 
%     % (see Section \ref{sec: quasi_newton} in the Appendix)
%     to get the approximation of the Hessian-vector product, $\B_{t}\textbf{v}$
    
%     \STATE Approximate $\nabla F\left(\w_{t}^{(k+1)};\miniB_t - \mathcal{R}^{(k)}\right)$ by: $\nabla F\left(\w_{t}^{(k+1)};\miniB_t - \mathcal{R}^{(k)}\right)= \nabla F\left(\w_{t}^{(k+1)};\miniB_t- \mathcal{R}^{(k)}\right) + \B_{t}\left(\w_{t}^{(k+1)} - \w_{t}^{(k)}\right)$
    
%     \STATE Compute $\w_{t+1}^{(k)}$ by using the "leave-$r$-out" gradient formula, based on the approximated $\nabla F(\w_{t}^{(k)}; \miniB_t)$ 
% }
% \ENDIF
% }
% \ENDFOR
% \STATE \textbf{Return} $\w_{T}^{(k+1)}$
% \end{algorithmic}
% \caption{\deltagradl}
% \label{alg: deltagradl}
% \end{algorithm}


At the $k_{th}$ round of loop \encircle{2}, after the human annotators clean the labels for a set of $b$ influential training samples, $\mathcal{R}^{(k)}$,
provided by the {Sample selector}, the next step is to update the model parameters in the {Model constructor}. To reduce the overhead of this step, we can regard the process of updating labels as two sub-processes, i.e. the deletions of the training samples, $\mathcal{R}^{(k)}$ (with the associated weight, $\gamma$), and the additions of those training samples with the cleaned labels (with the updated weight, 1), thus facilitating the use of \deltagrad. Specifically, the following modifications to Equation \eqref{eq: updated_gradient} are required: 1) the input deleted training samples should be $\mathcal{R}^{(k)}$; 2) the input cached model parameters and the corresponding gradients become the ones obtained at the $k-1_{st}$ round of the loop \encircle{2}; 3) instead of randomly sampling a mini-batch $\mathcal{A}_t$ from the added training samples $\mathcal{A}$, $\mathcal{A}_t$ should be replaced with the removed training samples from $\miniB_t$, i.e., $\miniB_t \bigcap \mathcal{R}^{(k)}$, but with updated labels; 4) the cleaned training samples and the uncleaned training samples so far are weighted by 1 and $\gamma$ respectively (this only slightly modifies how the loss is calculated for each mini-batch). Recall that in \deltagrad, there are three hyper-parameters, i.e. the number of ``burn-in'' iterations, $j_0$, the period, $T_0$, and the history size, $m_0$, which are thus also essential for \deltagradl.
% As mentioned in Section \ref{sec: intro}, we adjusted the solution, \deltagrad\ from \cite{wu2020deltagrad} for {\em incrementally} updating the models at each iteration of the loop \encircle{2}. 

% \subsection{\deltagradg}
\subsection{The human annotation phase}\label{sec: sample_cleaner}
As discussed in Section \ref{sec: intro}, the Sample selector not only suggests which samples should be cleaned, but also suggests the candidate cleaned labels, which can be regarded as one independent label annotator. When multiple annotators exist, we 
aggregate their labels by using majority vote to resolve possible label conflicts.
% aggregate those labels with the cleaned labels provided by the human annotators and thus produce the final cleaned labels, we use majority vote to resolve possible label conflicts. 

\textbf{Discussion} Note that indeed, only \deltagradl\ and \deltagradg\ explicitly rely on the strong convexity assumption on the model class. In contrast, \infl\ is potentially applicable for general machine learning models. Hence, we also conduct some initial experiments to evaluate the performance of \infl\ when neural network models are used in the extended technical report \cite{wu2021chef}.
% in Hence, we further  to evaluate the performance of \infl\ when convolutional neural networks (CNNs) are used 
% , which are presented in .
% % the Appendix \ref{sec: exp_cnn_model}. 
% The results also demonstrate the performance advantage of \infl\ in such general settings.

\eat{
\subsection{System overview}
Finally, we summarized the overview of the workflows in Algorithm \ref{alg: system}.

\begin{algorithm}
\small
 \caption{The workflow overview}\label{alg: system}
 \begin{spacing}{1}
 \begin{flushleft}
 \hspace*{\algorithmicindent}
 \textbf{Input:} The input model parameter: $\w^{(0)}$; The sequence of model parameters $\{\w^{(0)}_0, \w^{(0)}_1, \dots, \w^{(0)}_T\}$ and the corresponding mini-batches $\{\miniB_0, \miniB_1, \dots, \miniB_T\}$; The training set: $\mathcal{Z}$; a set of training samples with uncertain labels: $\mathcal{Z}^{(0)}$ (Note that $\mathcal{Z}^{(0)} \subset \mathcal{Z}$);  the validation set: $\mathcal{Z}_{\text{val}}$; the number of cleaning round in the loop \encircle{2}: $K$, the number of classes: $C$; the cleaning budget at each cleaning round: $b$\\
%  the Hessian-vector product: $\textbf{v}$; a set of training samples with uncertain labels: $\mathcal{Z}_{U}$; the validation dataset: $\mathcal{Z}_{\text{val}}$; the L2-norm of the class-wise hessian matrix derived at the $0_{th}$ round: $\{\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|\}_{j=1}^C$ for each $\z \in \mathcal{Z}_{U}$; the class-wise gradient: $\nabla_{\y}\nabla_\w F(\w^{(0)},\z)$ for each $\z \in \mathcal{Z}_{U}$; the cleaning budget at the current round: $b$ \\
\hspace*{\algorithmicindent} \textbf{Output:} Updated training set: $\mathcal{Z}$, the updated model: $\w^{(K)}$\\
\end{flushleft}
 \begin{algorithmic}[1]
\STATE \COMMENT{\textit{The initialization step below}} 
\STATE Pre-compute $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$ for each $\z = (\x,\y) \in \mathcal{Z}^{(0)}$ and for each class $j (j=1,2,\dots, C)$ by using Algorithm \ref{alg: pre_deltagrad}
\STATE Pre-compute the class-wise gradient $\nabla_{\y}\nabla_\w F(\w^{(0)},\z)$ for each $\z \in \mathcal{Z}^{(0)}$
% \STATE Initialize a list, $Infl=[]$, to contain the influence of each training sample with all deterministic labels
% \STATE Initialize two lists, $zl=[]$ and $yl=[]$, to contain the Top-$b$ influential training samples and suggested deterministic labels for them

\STATE In the {\em Sample selector}, invoke Algorithm \ref{alg: infl} on $\mathcal{Z}$ to obtain the Top-$b$ influential training samples $zl$ and the corresponding suggested labels $yl$, which are provided to the human annotators for cleaning
\FOR{k=0 to K-1}
\STATE After the cleaning process, update $\mathcal{Z}$ by replacing the labels of all the samples in $zl$ with the cleaned labels
\STATE Set $\mathcal{Z}^{(k+1)} = \mathcal{Z}^{(k)} - zl$ to represent the set of training samples with uncertain labels after the initialization step
\STATE In the {\em Model constructor}, compute the updated model $\w^{(k+1)}$ by invoking \deltagradl\ and obtain the sequence of model parameters during the training phase, $\{\w^{(k+1)}_0, \w^{(k+1)}_1,\dots, \w^{(k+1)}_T\}$
\IF{$k < K-1$}
{
\STATE In the {\em Sample selector}, invoke Algorithm \ref{alg: deltagradg} to obtain a set of candidate influential training samples $\mathcal{Z}^{(k+1)}_{inf}$
\STATE Invoke Algorithm \ref{alg: infl} on $\mathcal{Z}^{(k+1)}_{inf}$ to obtain the Top-$b$ influential training samples $zl$ and the corresponding suggested labels $yl$, which are provided to the human annotators for cleaning
}
\ENDIF
% apply \infl, i.e., Equation \eqref{eq: our_influence}, to compute the influence for each training sample $\z \in \mathcal{Z}^{(0)}$ with all possible deterministic labels $j=1,2,\dots, C$ if the label of $\z$ is uncertain, which is appended to $Infl$
% \STATE Sort $Infl$ in the {\em Sample selector} in ascending order and iterate through the sorted $Infl$ to 
\ENDFOR
% \STATE Initialize two lists $LB=[], UB=[]$, representing the lower bound and upper bound of the influence of each sample.
% \STATE Initialize one list $Infl=[]$ to include the value of $\pcenter$ for all $\z \in \mathcal{Z}_U$
% % \STATE Calculate $\textbf{v}=-\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)})$ by using the Hessian-vector product algorithm from \cite{koh2017understanding}.
%   % I want the below text to be left 
%   % "Some text before the logic:"
%   \FOR{each $\z \in \mathcal{Z}_{U}$}
%   \FOR{each deterministic label $c \in \{1,2,\dots, C\}$}
%     \STATE Denote $\delta_y = y - onehot(c)$
%     \STATE Calculate $\pcenter^{(k)}(\z, \delta_y)$ and add the result to the list $Infl$
%      \STATE Calculate the upper bound and lower bound of $\mathcal{I}^{(k)}_{\text{pert}}(\z, \mathcal{Z}_{\text{val}},\delta_y)$ % (denoted as $lb(\z,\delta_y)$ and $ub(\z,\delta_y)$) 
%      by using Theorem \ref{theorem: bound_influence} and add them to $UB$ and $LB$ respectively
%      \ENDFOR
%   \ENDFOR 
%     \STATE sort $Infl$ in ascending order, (denoted by $[\pcenter_1, \pcenter_2,\pcenter_3, \dots]$, add the corresponding training samples of the first $b$ entries in this sorted list to $\mathcal{Z}^{(k)}_{inf}$ and obtain their largest upper bound $L$
%     % \STATE 
%     \STATE For the remaining training samples, if the lower bound of their influence is smaller than $L$ with a certain $\delta_y$, add them to $\mathcal{Z}^{(k)}_{inf}$
%     % , which have one entry in $sInfl$ whose lower bound is larger than the upper bound of at least one entry within the first $b$ entries.
%     \STATE \textbf{Return} $\mathcal{Z}^{(k)}_{inf}$%and $\textbf{v}$.
  % I want the below text to be left 
%   \algotext{Some text before the logic:}

  % Here I want the numbering to start from 1 again
  \end{algorithmic}
  \end{spacing}
  \end{algorithm}



% \begin{algorithm}
% \small
%  \caption{Overview of our system}
%  \begin{spacing}{1}
%  \begin{flushleft}
%  \hspace*{\algorithmicindent}
%  \textbf{Input:} A training sample $\z \in \mathcal{Z}$, the class $j$ and the model parameter obtained in the initialization step: $\w^{(0)}$\\
% \hspace*{\algorithmicindent} \textbf{Output:} $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$. 
% \end{flushleft}
%  \begin{algorithmic}[1]
 
 
 
% % \STATE Initialize $\mathcal{Z}^{(k)}_{inf} = \{\}$
% % \STATE Initialize two lists $LB=[], UB=[]$, representing the lower bound and upper bound of the influence of each sample.
% % \STATE Initialize one list $Infl=[]$ to include the value of $\textbf{v}\nabla_{\y}\nabla_\w F(\w^{(0)},\z)\delta_{y}$ for all the sample $\z in \mathcal{Z}_U$
% % \STATE Calculate $\textbf{v}=-\nabla_\w F(\w^{(k)},\mathcal{Z}_{\text{val}})^\top \bH^{-1}(\w^{(k)})$ by using the Hessian-vector product algorithm from \cite{koh2017understanding}.
%   % I want the below text to be left 
%   % "Some text before the logic:"
% %   \FOR{each $\z \in \mathcal{Z}$}
%     \STATE 
%   \STATE Initialization step: pre-compute  $\textbf{g}$ as a random vector;
%   \STATE \COMMENT{\textit{Power method below}}
%   \WHILE{\textbf{g} is not converged} 
%     \STATE Calculate $-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\textbf{g}$ by using Equation \eqref{eq: hessian_vector_prod}
%     \STATE Update $\textbf{g}$: $\textbf{g}=\frac{-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\textbf{g}}{\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\textbf{g}\|}$
%   \ENDWHILE 
%   \STATE Calculate the largest eigenvalue of $-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))$ in magnitude by using $ \frac{\textbf{g}\cdot (-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\textbf{g})}{\|\textbf{g}\|}$, which is equivalent to $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$.
% %   \FOR{each deterministic label $c \in \{1,2,\dots, C\}$}
% %     \STATE Denote $\delta_y = y - onehot(c)$
% %     \STATE Calculate $\textbf{v}\nabla_{\y}\nabla_\w F(\w^{(0)},\z)\delta_{y}$ and add the result to the list $Infl$
% %      \STATE Calculate the upper bound and lower bound of $\mathcal{I}^{(k)}_{\text{pert}}(\z, \mathcal{Z}_{\text{val}},\delta_y)$ (denoted as $lb(\z,\delta_y)$ and $ub(\z,\delta_y)$) by using Theorem \ref{theorem: bound_influence}.
% %      Add $lb(\z,\delta_y)$ to $LB$ and add $ub(\z,\delta_y)$ to $UB$
% %      \ENDFOR
% %   \ENDFOR 
%     % \STATE sort $Infl$ in ascending order and denote the sorted list as $sInfl$
%     % \STATE For the first $b$ entries in $sInfl$, add the corresponding training samples to $\mathcal{Z}^{(k)}_{inf}$
%     % \STATE For the remaining entries in $sInfl$, add the training samples to $\mathcal{Z}^{(k)}_{inf}$, which have one entry in $sInfl$ whose lower bound is larger than the upper bound of at least one entry within the first $b$ entries.
%     \STATE \textbf{Return} $\|-\nabla_{\w}^2\log(p^{(j)}(\w^{(0)}, \x))\|$.
%   % I want the below text to be left 
% %   \algotext{Some text before the logic:}

%   % Here I want the numbering to start from 1 again
%   \end{algorithmic}
%   \end{spacing}
%   \end{algorithm}
% \begin{algorithm}[H] 
% \small
% % \footnotesize
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \Input{The model parameter used for selecting the influential training sample at the $k_{th}$ iteration, $\w^{(k)}$; training samples with uncertain labels, $\mathcal{Z}_{U}$; the class-wise hessian matrix  $-\nabla_{\w}^2\log(p^{(r)}(\w^{(0)}, \x))$; the class-wise gradient $\nabla_{\y}\nabla_\w F(\w^{(0)},\z)$ and the number of training samples to be cleaned, $k$}
% \Output{A set of prioritized training samples for cleaning $\mathcal{Z}^{(k)}_{inf}$}




% Initialize $\mathcal{Z}^{(k)}_{inf} = \{\}$

% \For{$\z \in \mathcal{Z}_{U}$}{


% }


% % Initialize an array $\Delta G = \left[\right]$

% % Initialize an array $\Delta W = \left[\right]$

% % \For{$t=0;t<T; t++$}{

% % \eIf{$[((t-j_0) \mod T_0) == 0]$ or $t \leq j_0$}
% % {
% %     compute $\nabla F\left(\iw_{t}\right)$ exactly
    
% %     compute $\nabla F\left(\iw_{t}\right) - \nabla F\left(\w_{t}\right)$ based on the cached gradient $\nabla F\left(\w_{t}\right)$
    
% %     set $\Delta G\left[k\right] = \nabla F\left(\iw_{t}\right) - \nabla F\left(\w_{t}\right)$
    
% %     set $\Delta W\left[k\right] = \iw_{t} - \w_{t}$, based on the cached parameters $\w_{t}$
    
% %     $k\leftarrow k+1$
    
% %     compute $\iw_{t+1}$ by using exact GD update (equation \eqref{eq: update_rule_naive})
% % }
% % {
% %     Pass $\Delta W\left[-m:\right]$, $\Delta G\left[-m:\right]$, the last $m$ elements in $\Delta W$ and $\Delta G$, which are from the $j_1^{th}, j_2^{th},\dots, j_m^{th}$ iterations where $j_1 < j_2< \dots < j_m$ depend on $t$, $\textbf{v} = \iw_{t} - \w_{t}$, and the history size $m$, to the L-BFGFS Algorithm (see Section \ref{sec: quasi_newton} in the Appendix) to get the approximation of $\bH(\w_{t})\textbf{v}$, i.e., $\B_{j_m}\textbf{v}$
    
% %     Approximate $\nabla F\left(\iw_{t}\right) = \nabla F\left(\w_{t}\right) + \B_{j_m}\left(\iw_{t} - \w_{t}\right)$
    
% %     Compute $\iw_{t+1}$ by using the "leave-$r$-out" gradient formula, based on the approximated $\nabla F(\iw_{t})$ 
% % }
% % }

% \Return $\w_{t}$
% \caption{\infl}
% \label{alg: infl}
}% \end{algorithm}
